Matrix Perturbation Theory in the Tangent Space of Isospectral Matrices

Eigenvalue and eigenvector perturbation theory is a fundamental topic in several disciplines, including numerical linear algebra, quantum physics, and related fields. The central problem is to understand how the eigenvalues and eigenvectors of a matrix $A \in \mathbb{C}^{n \times n}$ change under the addition of a perturbation matrix $E \in \mathbb{C}^{n \times n}$. Much of the existing literature focuses on structured perturbations. For example, in [C.-K. Li and R.-C. Li, Linear Algebra Appl. 2005], the matrix $A$ is assumed to be Hermitian and block diagonal, while the perturbation $E$ is Hermitian and block off-diagonal. In this work, we investigate a different structured setting in which the perturbation has the commutator form $E = AB - BA$ for some matrix $B$, which we show to be a generalization of the block diagonal structure considered by Li and Li. First, we extend their main result by showing that the perturbation of the $i$-th eigenvalue of $A$, denoted by $\lambda_i$, is of order $\|E\|^2 / \eta_i$, where $\eta_i = \min_{j \neq i} |\lambda_i - \lambda_j|$ is the spectral gap associated with $\lambda_i$. Second, we provide a detailed analysis of the role played by the matrix $B$ in the perturbation of the eigenvectors. This analysis is further generalized to the case of block-diagonal matrices with multiple eigenvalues, as well as to perturbed singular values and eigenvalues of Jordan blocks.

==> experiments/blockequiherm.tex <==
n err bound
1	2.38683938968769e-12	1.65840364780952e-10
2	2.01411489224441e-12	1.65840364780952e-10
3	2.01411489224441e-12	1.65840364780952e-10
4	2.27442008385234e-12	1.65840364780952e-10
5	2.27442008385234e-12	1.65840364780952e-10
6	1.29262892434990e-12	1.65840364780952e-10
7	1.17950988271643e-12	1.65840364780952e-10
8	1.17950988271643e-12	1.65840364780952e-10
9	9.89100603728694e-13	1.65840364780952e-10
10	9.89100603728694e-13	1.65840364780952e-10
11	1.70852307327538e-12	1.65840364780952e-10
12	1.70852307327538e-12	1.65840364780952e-10
13	1.25275320173541e-12	1.65840364780952e-10
14	1.03561850668759e-12	1.65840364780952e-10
15	1.03561850668759e-12	1.65840364780952e-10
16	1.80906102550802e-12	1.65840364780952e-10
17	1.80906102550802e-12	1.65840364780952e-10
18	2.67382348642875e-12	1.65840364780952e-10
19	2.67382348642875e-12	1.65840364780952e-10
20	7.44702521736399e-13	1.65840364780952e-10
21	7.44702521736399e-13	1.65840364780952e-10
22	8.69960100360215e-13	1.65840364780952e-10
23	8.69960100360215e-13	1.65840364780952e-10
24	7.11193694264599e-13	1.65840364780952e-10
25	7.11193694264599e-13	1.65840364780952e-10
26	8.01340824614669e-13	1.65840364780952e-10
27	8.01340824614669e-13	1.65840364780952e-10
28	3.67825122241027e-13	1.65840364780952e-10
29	3.67825122241027e-13	1.65840364780952e-10
30	1.82036241056543e-13	1.65840364780952e-10
31	1.38911284447697e-12	1.65840364780952e-10
32	1.38911284447697e-12	1.65840364780952e-10
33	1.06054072410450e-12	1.65840364780952e-10
34	1.06054072410450e-12	1.65840364780952e-10
35	1.80772306501851e-13	1.65840364780952e-10
36	3.14030639265112e-13	1.65840364780952e-10
37	3.14030639265112e-13	1.65840364780952e-10
38	1.17568980195466e-13	1.65840364780952e-10
39	1.17568980195466e-13	1.65840364780952e-10
40	1.31649845610119e-13	1.65840364780952e-10
41	1.31649845610119e-13	1.65840364780952e-10
42	9.39461498448766e-13	1.65840364780952e-10
43	9.39461498448766e-13	1.65840364780952e-10
44	2.45771382473734e-13	1.65840364780952e-10
45	2.45771382473734e-13	1.65840364780952e-10
46	9.46719861035355e-14	1.65840364780952e-10
47	9.46719861035355e-14	1.65840364780952e-10
48	1.02443956184899e-14	1.65840364780952e-10
49	1.02443956184899e-14	1.65840364780952e-10
50	2.39031994046337e-14	1.65840364780952e-10
51	2.39031994046337e-14	1.65840364780952e-10
52	2.18207929742674e-15	1.65840364780952e-10
53	4.92993814553498e-15	1.65840364780952e-10
54	4.92993814553498e-15	1.65840364780952e-10
55	4.41097570110851e-13	1.65840364780952e-10
56	4.41097570110851e-13	1.65840364780952e-10
57	6.48445626888673e-14	1.65840364780952e-10
58	6.48445626888673e-14	1.65840364780952e-10
59	1.08065231129732e-13	1.65840364780952e-10
60	1.08065231129732e-13	1.65840364780952e-10
61	1.32720346155883e-13	1.65840364780952e-10
62	1.32720346155883e-13	1.65840364780952e-10
63	4.01919418724439e-13	1.65840364780952e-10
64	4.01919418724439e-13	1.65840364780952e-10
65	8.77264893905379e-13	1.65840364780952e-10
66	8.77264893905379e-13	1.65840364780952e-10
67	1.60560264399595e-13	1.65840364780952e-10
68	1.60560264399595e-13	1.65840364780952e-10
69	5.90015055707733e-13	1.65840364780952e-10
70	5.90015055707733e-13	1.65840364780952e-10
71	1.40277674573471e-12	1.65840364780952e-10
72	1.40277674573471e-12	1.65840364780952e-10
73	7.07965134072107e-13	1.65840364780952e-10
74	7.07965134072107e-13	1.65840364780952e-10
75	1.83703396546560e-13	1.65840364780952e-10
76	5.19132074356323e-13	1.65840364780952e-10
77	8.65650479045880e-13	1.65840364780952e-10
78	8.65650479045880e-13	1.65840364780952e-10
79	1.99226721335583e-12	1.65840364780952e-10
80	1.99226721335583e-12	1.65840364780952e-10
81	8.68564306562315e-13	1.65840364780952e-10
82	8.68564306562315e-13	1.65840364780952e-10
83	4.54032944038884e-13	1.65840364780952e-10
84	4.54032944038884e-13	1.65840364780952e-10
85	5.74722327624898e-13	1.65840364780952e-10
86	1.79834853177856e-12	1.65840364780952e-10
87	1.51868486389175e-12	1.65840364780952e-10
88	1.51868486389175e-12	1.65840364780952e-10
89	1.63177274060193e-12	1.65840364780952e-10
90	2.66011499830360e-12	1.65840364780952e-10
91	2.66011499830360e-12	1.65840364780952e-10
92	1.31631492427823e-12	1.65840364780952e-10
93	1.31631492427823e-12	1.65840364780952e-10
94	1.44148623261443e-12	1.65840364780952e-10
95	2.70142547853278e-12	1.65840364780952e-10
96	2.70142547853278e-12	1.65840364780952e-10
97	1.48346551813062e-12	1.65840364780952e-10
98	1.48346551813062e-12	1.65840364780952e-10
99	2.63437066213554e-12	1.65840364780952e-10
100	2.63437066213554e-12	1.65840364780952e-10

==> experiments/cubicequi.tex <==
n err bound boundsharp
1	2.65194949428677e-14	2.00735640220293e-09	1.16271347471095e-11
2	7.51217124953432e-14	2.00735640220293e-09	1.10280225518420e-11
3	7.74512699040638e-14	2.00735640220293e-09	1.04701428178240e-11
4	7.57576134067383e-14	2.00735640220293e-09	1.19966498345034e-11
5	4.73886490644882e-14	2.00735640220293e-09	1.03814435179870e-11
6	6.32233608029878e-14	2.00735640220293e-09	1.07698589463336e-11
7	8.63527636623498e-14	2.00735640220293e-09	1.03290400332311e-11
8	7.81637345516874e-14	2.00735640220293e-09	1.12157635171297e-11
9	4.28309033815826e-14	2.00735640220293e-09	1.06231773109657e-11
10	6.17816011720030e-14	2.00735640220293e-09	1.14826225398022e-11
11	5.74351443103333e-14	2.00735640220293e-09	1.14789992547140e-11
12	5.93071216415560e-14	2.00735640220293e-09	1.05137515863304e-11
13	5.18432386670899e-14	2.00735640220293e-09	1.05646079486523e-11
14	6.26885394886997e-14	2.00735640220293e-09	1.15969024264361e-11
15	1.27774002613878e-13	2.00735640220293e-09	1.13114097884816e-11
16	1.20537629463159e-13	2.00735640220293e-09	1.09348607990931e-11
17	5.39202764122820e-14	2.00735640220293e-09	1.06067587886594e-11
18	5.13892567833331e-14	2.00735640220293e-09	1.09242506739645e-11
19	6.14221830394972e-14	2.00735640220293e-09	1.15613861846573e-11
20	6.21656398109503e-14	2.00735640220293e-09	1.01751610348039e-11
21	2.16242210656423e-14	2.00735640220293e-09	1.09678681721929e-11
22	4.19421794244619e-14	2.00735640220293e-09	1.13164861792491e-11
23	8.43532578943261e-14	2.00735640220293e-09	1.12095656397566e-11
24	5.47474656352801e-14	2.00735640220293e-09	1.11973534585045e-11
25	5.08404354763201e-14	2.00735640220293e-09	1.16905415392318e-11
26	3.28057447361116e-14	2.00735640220293e-09	1.10147528448194e-11
27	3.53589377317944e-14	2.00735640220293e-09	1.04752015228330e-11
28	5.32192113234219e-14	2.00735640220293e-09	1.04907321153421e-11
29	3.54380182316195e-14	2.00735640220293e-09	1.05030905608697e-11
30	9.71040511284186e-14	2.00735640220293e-09	1.10998110183062e-11
31	8.53296401126484e-14	2.00735640220293e-09	1.10324936695555e-11
32	7.31704171213410e-14	2.00735640220293e-09	1.11531310949155e-11
33	8.62205928234881e-14	2.00735640220293e-09	1.13026246245621e-11
34	8.30921714004890e-14	2.00735640220293e-09	9.99146001604382e-12
35	1.27382797456135e-13	2.00735640220293e-09	1.10653073778459e-11
36	1.19045368031132e-13	2.00735640220293e-09	1.05142891184348e-11
37	6.06465279271146e-14	2.00735640220293e-09	1.18640669959087e-11
38	8.65476284751709e-14	2.00735640220293e-09	1.14330243210479e-11
39	6.30813478343857e-14	2.00735640220293e-09	1.11463941947210e-11
40	6.61112751281174e-14	2.00735640220293e-09	1.10516239419613e-11
41	6.08102919128944e-14	2.00735640220293e-09	1.11591692344579e-11
42	6.66896393486153e-14	2.00735640220293e-09	1.03387749942233e-11
43	1.66800633887130e-13	2.00735640220293e-09	1.21337725455701e-11
44	1.96289008525597e-13	2.00735640220293e-09	1.01233980324661e-11
45	9.83674053804465e-14	2.00735640220293e-09	1.10360713694166e-11
46	5.04917343702748e-14	2.00735640220293e-09	1.11810780833833e-11
47	7.97799587120889e-14	2.00735640220293e-09	1.13104245362399e-11
48	1.93194713563334e-13	2.00735640220293e-09	1.08193056677255e-11
49	1.16582019703631e-13	2.00735640220293e-09	9.55883115893142e-12
50	7.86600849232161e-14	2.00735640220293e-09	1.13977051027966e-11
51	7.44288174779542e-14	2.00735640220293e-09	1.09154413903367e-11
52	4.46506101491858e-14	2.00735640220293e-09	1.07730538898429e-11
53	1.71733111359613e-13	2.00735640220293e-09	1.13155531462395e-11
54	1.99013454506710e-13	2.00735640220293e-09	1.12001847737817e-11
55	4.16844121102506e-14	2.00735640220293e-09	1.17608529523122e-11
56	2.93712902221297e-14	2.00735640220293e-09	1.05080546303052e-11
57	1.66448634632771e-13	2.00735640220293e-09	1.07212771821118e-11
58	1.78918836837713e-13	2.00735640220293e-09	1.20889150071491e-11
59	1.17602310898664e-13	2.00735640220293e-09	1.13981408198914e-11
60	9.74575170025503e-14	2.00735640220293e-09	1.14598443549781e-11
61	5.98373309435664e-14	2.00735640220293e-09	1.00557395926354e-11
62	8.58258599294598e-14	2.00735640220293e-09	1.02390845877589e-11
63	1.04710665349326e-13	2.00735640220293e-09	1.03027411486586e-11
64	1.02286874222846e-13	2.00735640220293e-09	1.05951940393290e-11
65	4.78860816842118e-14	2.00735640220293e-09	1.06555782097820e-11
66	4.75646648707887e-14	2.00735640220293e-09	1.11881372475826e-11
67	8.80291090644826e-14	2.00735640220293e-09	1.11747992624263e-11
68	1.95151428147660e-13	2.00735640220293e-09	1.14981601529136e-11
69	1.78669970157024e-13	2.00735640220293e-09	1.07386386910418e-11
70	1.04454062473215e-13	2.00735640220293e-09	9.87980557194534e-12
71	1.25095846543862e-13	2.00735640220293e-09	1.15876380926468e-11
72	2.33003401698828e-14	2.00735640220293e-09	1.19734258510234e-11
73	1.27477593740449e-13	2.00735640220293e-09	1.05448803748408e-11
74	1.54107506993473e-13	2.00735640220293e-09	1.12986941975059e-11
75	1.45713618571553e-13	2.00735640220293e-09	1.14464732214002e-11
76	1.51080050978089e-13	2.00735640220293e-09	1.13943378419711e-11
77	4.26675435315871e-14	2.00735640220293e-09	9.67106450944626e-12
78	3.00976693998290e-13	2.00735640220293e-09	1.22559979379878e-11
79	3.78086349210286e-13	2.00735640220293e-09	1.10580487658729e-11
80	2.74678205597815e-13	2.00735640220293e-09	1.16100949420509e-11
81	1.30135981355447e-13	2.00735640220293e-09	1.05399531535906e-11
82	5.56721226210390e-14	2.00735640220293e-09	1.07833559358108e-11
83	5.37656625208378e-14	2.00735640220293e-09	1.06307015305903e-11
84	8.96951214401723e-14	2.00735640220293e-09	1.08214978505021e-11
85	5.84688953936501e-14	2.00735640220293e-09	1.15486636912793e-11
86	1.32489883198328e-13	2.00735640220293e-09	1.06190040329279e-11
87	3.27205094797877e-14	2.00735640220293e-09	1.05210302302594e-11
88	8.91799509527408e-14	2.00735640220293e-09	1.04215631663157e-11
89	4.65023015445337e-14	2.00735640220293e-09	1.09334784401900e-11
90	1.04873401563946e-13	2.00735640220293e-09	1.06878256253043e-11
91	6.77736856180574e-14	2.00735640220293e-09	1.07218446292629e-11
92	4.78274760878837e-14	2.00735640220293e-09	1.12566867733835e-11
93	8.05088719420518e-14	2.00735640220293e-09	1.19939035420166e-11
94	1.13066789949912e-13	2.00735640220293e-09	1.08379592717948e-11
95	1.91972578105166e-13	2.00735640220293e-09	1.14515274743232e-11
96	1.44377731123739e-13	2.00735640220293e-09	1.07607056389057e-11
97	1.06324133985184e-13	2.00735640220293e-09	1.14811666345497e-11
98	6.97266390292922e-14	2.00735640220293e-09	1.10466752098433e-11
99	4.54271411886156e-14	2.00735640220293e-09	1.11991410938834e-11
100	4.43372402556496e-14	2.00735640220293e-09	1.13343706664804e-11
101	3.76847717906473e-14	2.00735640220293e-09	1.13669949216469e-11
102	7.69917967973795e-14	2.00735640220293e-09	1.09487408970958e-11
103	8.33432743953000e-14	2.00735640220293e-09	1.03758047454438e-11
104	9.38123211144303e-14	2.00735640220293e-09	1.10468994095934e-11
105	8.64682015211916e-14	2.00735640220293e-09	1.02473718360506e-11
106	1.10724188937387e-13	2.00735640220293e-09	1.13160770622477e-11
107	3.87228956254507e-14	2.00735640220293e-09	1.09641236585432e-11
108	3.37589643818070e-13	2.00735640220293e-09	1.13624882501236e-11
109	3.04295046462825e-13	2.00735640220293e-09	1.03722085664911e-11
110	3.44207771349224e-14	2.00735640220293e-09	1.02349991605567e-11
111	7.02794073403863e-14	2.00735640220293e-09	1.15858647485856e-11
112	1.21565552159065e-13	2.00735640220293e-09	1.19157759847752e-11
113	8.14273858612512e-14	2.00735640220293e-09	1.02862807969970e-11
114	6.01357889222614e-14	2.00735640220293e-09	1.11490978090277e-11
115	1.10811624549984e-13	2.00735640220293e-09	1.20900914177148e-11
116	1.68634438807429e-13	2.00735640220293e-09	1.21962732434923e-11
117	1.57217222555275e-13	2.00735640220293e-09	1.22603288691995e-11
118	3.84607798896842e-13	2.00735640220293e-09	1.13055701995701e-11
119	4.09332877733615e-13	2.00735640220293e-09	1.01209077934720e-11
120	1.69632612942860e-13	2.00735640220293e-09	1.14666261647341e-11
121	1.11963176558256e-13	2.00735640220293e-09	1.18325907006034e-11
122	3.83228617731455e-14	2.00735640220293e-09	1.12626747782749e-11
123	1.04499730512083e-13	2.00735640220293e-09	1.23476447389694e-11
124	6.13604828971920e-14	2.00735640220293e-09	1.10954154142563e-11
125	1.01164918205577e-13	2.00735640220293e-09	1.08853574254077e-11
126	5.87747660044696e-14	2.00735640220293e-09	1.15031804935203e-11
127	6.97697364091309e-14	2.00735640220293e-09	1.12496839829369e-11
128	7.32968699098058e-14	2.00735640220293e-09	1.11535766744151e-11
129	8.08816141128930e-14	2.00735640220293e-09	1.11431482669598e-11
130	9.54865836419454e-14	2.00735640220293e-09	1.14817605349062e-11
131	8.77377800710881e-14	2.00735640220293e-09	1.14342415005812e-11
132	1.11034439456762e-13	2.00735640220293e-09	1.09658219075435e-11
133	2.44945913544926e-13	2.00735640220293e-09	1.13358667414847e-11
134	6.49239972734095e-14	2.00735640220293e-09	1.02341898381827e-11
135	2.02467689472423e-13	2.00735640220293e-09	1.13649773327537e-11
136	2.98431281688124e-13	2.00735640220293e-09	1.06373082633918e-11
137	2.29751368472018e-13	2.00735640220293e-09	1.10301568165619e-11
138	2.43014888041573e-13	2.00735640220293e-09	1.10720583095953e-11
139	2.04846684666174e-13	2.00735640220293e-09	1.11021970059925e-11
140	2.59528679168352e-13	2.00735640220293e-09	1.18868154959381e-11
141	1.90284188511305e-13	2.00735640220293e-09	1.09768075296335e-11
142	1.33374212589510e-13	2.00735640220293e-09	1.15246629840837e-11
143	2.00612642485959e-13	2.00735640220293e-09	1.09309500325058e-11
144	1.98341083229360e-13	2.00735640220293e-09	1.05162674979240e-11
145	1.45358556179520e-13	2.00735640220293e-09	1.12669621902195e-11
146	5.36193627882828e-13	2.00735640220293e-09	1.08245108379427e-11
147	5.18359754288229e-13	2.00735640220293e-09	1.13460299366489e-11
148	7.25194798093396e-14	2.00735640220293e-09	1.16980636792878e-11
149	9.37268163674458e-14	2.00735640220293e-09	1.18754527517906e-11
150	8.81285747560191e-14	2.00735640220293e-09	1.08627960695057e-11
151	1.98353018157670e-13	2.00735640220293e-09	1.19678456492302e-11
152	1.84802038778748e-13	2.00735640220293e-09	1.11981732149848e-11
153	1.54621191249751e-13	2.00735640220293e-09	1.04292782008680e-11
154	1.34478374799469e-13	2.00735640220293e-09	1.16150339304242e-11
155	1.23275027968866e-13	2.00735640220293e-09	1.11001912529932e-11
156	1.39799506860221e-13	2.00735640220293e-09	1.07122248602199e-11
157	1.81253442811907e-13	2.00735640220293e-09	1.12500938278048e-11
158	9.82233777136306e-14	2.00735640220293e-09	1.16990616775669e-11
159	1.36097809817959e-13	2.00735640220293e-09	1.16475015442154e-11
160	6.36489940250898e-14	2.00735640220293e-09	1.07290322055046e-11
161	1.99186011075343e-13	2.00735640220293e-09	1.13385676418173e-11
162	1.77253762649615e-13	2.00735640220293e-09	1.04807169199156e-11
163	2.34948525552523e-13	2.00735640220293e-09	1.15500565224895e-11
164	2.13756327938500e-13	2.00735640220293e-09	1.21935196558144e-11
165	3.27836617764046e-13	2.00735640220293e-09	1.07345445431008e-11
166	2.99257057792775e-13	2.00735640220293e-09	1.07098825607956e-11
167	1.08191214304734e-13	2.00735640220293e-09	1.11446221797730e-11
168	6.23458448335552e-14	2.00735640220293e-09	1.11509738747365e-11
169	7.01624470548534e-14	2.00735640220293e-09	1.12382384109813e-11
170	4.33691567171811e-13	2.00735640220293e-09	9.76768210447754e-12
171	2.46878121186693e-13	2.00735640220293e-09	1.07157988938662e-11
172	1.42695845109595e-13	2.00735640220293e-09	1.12102244028833e-11
173	1.44874676793734e-13	2.00735640220293e-09	1.13264726451414e-11
174	5.24058266822406e-13	2.00735640220293e-09	1.21393199848340e-11
175	4.83405417723766e-13	2.00735640220293e-09	1.07175475616131e-11
176	3.80072663755450e-13	2.00735640220293e-09	1.06939162534139e-11
177	4.41741079268508e-13	2.00735640220293e-09	1.06508732816708e-11
178	3.41153247841064e-13	2.00735640220293e-09	1.13837683236262e-11
179	2.70036239362092e-13	2.00735640220293e-09	1.11862531843043e-11
180	4.81024538329700e-13	2.00735640220293e-09	1.18949210542704e-11
181	6.47040454147306e-13	2.00735640220293e-09	1.08235177437999e-11
182	4.77486328995274e-13	2.00735640220293e-09	1.07758588184706e-11
183	4.81477272794380e-13	2.00735640220293e-09	1.10471971249340e-11
184	4.39302135730606e-13	2.00735640220293e-09	1.13301657304127e-11
185	1.19408347825385e-13	2.00735640220293e-09	1.07464031967839e-11
186	7.18055318537901e-13	2.00735640220293e-09	1.13031065252864e-11
187	8.23274243050983e-13	2.00735640220293e-09	1.06721778184906e-11
188	3.98364619785005e-13	2.00735640220293e-09	1.16990654338373e-11
189	1.42081953794836e-13	2.00735640220293e-09	1.01382283580423e-11
190	5.05499147786383e-13	2.00735640220293e-09	1.00557447812118e-11
191	6.08334704349543e-13	2.00735640220293e-09	1.11719560128185e-11
192	8.26848265476564e-13	2.00735640220293e-09	1.19152158362947e-11
193	8.12753916089058e-13	2.00735640220293e-09	1.15646908107508e-11
194	2.02710624477257e-13	2.00735640220293e-09	1.19675366178313e-11
195	2.03019994182038e-13	2.00735640220293e-09	1.06385086243397e-11
196	4.57703837972716e-13	2.00735640220293e-09	1.10231893246919e-11
197	4.18442161505398e-13	2.00735640220293e-09	1.16114366277662e-11
198	2.97091764014546e-13	2.00735640220293e-09	1.09099723612580e-11
199	2.71485021009856e-13	2.00735640220293e-09	1.15531331297957e-11
200	1.11388490419748e-13	2.00735640220293e-09	1.16305348568053e-11

==> experiments/cubicpow2.tex <==
n err bound boundsharp
1	1.36402474526287e-12	0.00306069958847737	2.06234563127483e-07
2	8.49942497653260e-13	0.00306069958847737	2.44085275717954e-07
3	3.89102538702344e-13	0.000548816622986593	7.00087931460524e-08
4	6.14020186310163e-13	0.000185986479551777	3.29529117850312e-08
5	6.09817986487552e-13	8.41785263989870e-05	1.99136226180463e-08
6	2.24861647894656e-13	4.50058576988289e-05	1.12632244225310e-08
7	1.71034586847926e-13	2.68203859308594e-05	8.37954807107465e-09
8	1.68641666879732e-13	1.72516032031571e-05	6.50967897595643e-09
9	2.08735979592836e-13	1.17439968255754e-05	5.00847582829450e-09
10	1.33559911665281e-13	8.35235311221379e-06	3.92866065348110e-09
11	2.08557929198338e-13	6.15062616318272e-06	3.34006858396224e-09
12	1.00162566844907e-13	4.65953312720357e-06	2.63845350341182e-09
13	1.14253845075561e-13	3.61399968923171e-06	2.40589884087744e-09
14	1.16652950254958e-13	2.85928445658881e-06	1.94624614927817e-09
15	1.63035002775323e-13	2.30090817477496e-06	1.56071477936338e-09
16	1.32202112201890e-13	1.87895729676176e-06	1.58556600763744e-09
17	1.27908237464775e-13	1.55418520164443e-06	1.32151557646918e-09
18	7.02416200629969e-14	1.30015079025666e-06	1.09833354299671e-09
19	5.80295497784157e-14	1.09859718609580e-06	1.02337427933677e-09
20	6.36843850759817e-14	9.36642322598037e-07	9.17102420049141e-10
21	1.11555122638776e-13	8.05019817890765e-07	8.19579125161078e-10
22	8.80226685538229e-14	6.96948260133157e-07	7.25967695251714e-10
23	5.23976083051083e-14	6.07387219101406e-07	6.46707369432454e-10
24	1.01132900510399e-13	5.32537320420209e-07	6.70278478607951e-10
25	8.09359485233147e-14	4.69497879300156e-07	6.01158438828983e-10
26	7.24826614812989e-14	4.16028358580098e-07	5.53234415216380e-10
27	9.38435158149028e-14	3.70379530873462e-07	5.36151603547867e-10
28	5.66652218324465e-14	3.31172242358085e-07	4.47145393051129e-10
29	3.91767583867531e-14	2.97309196562456e-07	4.18510482376144e-10
30	8.50350315551072e-14	2.67909975383185e-07	3.88665507192383e-10
31	7.09323788556757e-14	2.42262631801195e-07	3.72943769547540e-10
32	6.52075417275773e-14	2.19787247272923e-07	3.67250032695742e-10
33	6.27529254545338e-14	2.00008227025776e-07	3.39766821876219e-10
34	2.72205028263660e-14	1.82533045156965e-07	2.95004268270989e-10
35	4.71173468719514e-14	1.67035798265942e-07	3.10093466354153e-10
36	6.31351058095482e-14	1.53244377594082e-07	2.67236393785932e-10
37	4.64807217060135e-14	1.40930388085956e-07	2.48841519041921e-10
38	2.83530894863660e-14	1.29901169946556e-07	2.47964561293465e-10
39	2.95165858979694e-14	1.19993441964687e-07	2.46799990606629e-10
40	5.20658586345215e-14	1.11068204965989e-07	2.25500211158318e-10
41	3.73303370093932e-14	1.03006631185981e-07	1.96373930439830e-10
42	3.15316806964006e-14	9.57067300818119e-08	1.90317936366072e-10
43	6.30097705681603e-14	8.90806294113508e-08	1.93139253171089e-10
44	5.09880912811350e-14	8.30523467402196e-08	1.80259340670076e-10
45	4.97479189037728e-14	7.75559540594566e-08	1.82007971421141e-10
46	7.31478763245005e-14	7.25340591887896e-08	1.53723777082520e-10
47	4.48536449023857e-14	6.79365437572194e-08	1.61049601929045e-10
48	3.71867326967832e-14	6.37195100034930e-08	1.53426897384914e-10
49	3.27964169353737e-14	5.98443983152014e-08	1.56289552150647e-10
50	3.91090175718077e-14	5.62772449878084e-08	1.40633213474017e-10
51	4.74046375685234e-14	5.29880556277177e-08	1.28858335182996e-10
52	4.00425035691307e-14	4.99502743177245e-08	1.31549120245452e-10
53	7.09669554447367e-14	4.71403323896686e-08	1.24949434424588e-10
54	6.94740133790484e-14	4.45372636214419e-08	1.23775035452672e-10
55	2.49073171596280e-14	4.21223750571809e-08	1.18409646404834e-10
56	3.93465089766751e-14	3.98789645662627e-08	1.05149756540077e-10
57	3.55748274846168e-14	3.77920778058774e-08	1.09194064077927e-10
58	1.91866308846643e-14	3.58482985090795e-08	1.09286814748973e-10
59	3.20482001617700e-14	3.40355670443542e-08	1.05340677807962e-10
60	3.42934450819920e-14	3.23430230302069e-08	9.35197169375137e-11
61	2.77359733020088e-14	3.07608684755968e-08	8.62422942710937e-11
62	4.00647484991474e-14	2.92802484830916e-08	9.68377950053124e-11
63	2.71777059967823e-14	2.78931470193847e-08	8.02178283338958e-11
64	8.77881391640346e-14	2.65922956456223e-08	8.58246381218714e-11
65	1.07152379930236e-13	2.53710934225110e-08	8.19661111841701e-11
66	5.82820541265403e-14	2.42235364742303e-08	8.54275432658135e-11
67	2.65330810930432e-14	2.31441559202825e-08	7.77557494174634e-11
68	1.90529001402939e-14	2.21279630732905e-08	7.78421476104704e-11
69	9.63066619562583e-14	2.11704009596698e-08	6.79416905479729e-11
70	1.15953006857774e-13	2.02673013541712e-08	7.31802301994159e-11
71	4.69324716309596e-14	1.94148466326840e-08	6.91629789962936e-11
72	6.38487428431962e-14	1.86095358438495e-08	6.39977071960048e-11
73	3.45420136973185e-14	1.78481544817624e-08	6.44301973925032e-11
74	1.17885921862819e-13	1.71277475116834e-08	6.04424713762023e-11
75	1.02017625729552e-13	1.64455952601576e-08	6.21392013334194e-11
76	5.58299692981086e-14	1.57991918318362e-08	5.60197215780562e-11
77	3.57497191577765e-14	1.51862257589648e-08	6.05606649896702e-11
78	5.87691983462703e-14	1.46045626270342e-08	5.49976766463272e-11
79	6.57576075917370e-14	1.40522294524200e-08	5.60391560970075e-11
80	8.83345523946826e-14	1.35274006157389e-08	5.41183501185286e-11
81	6.66189975578415e-14	1.30283851787825e-08	5.96960434723822e-11
82	6.85198368595503e-14	1.25536154337913e-08	5.50833234765548e-11
83	3.45970933509321e-14	1.21016365519850e-08	4.87294243973215e-11
84	4.09522275306199e-14	1.16710972140371e-08	5.23529032971612e-11
85	5.05050260100539e-14	1.12607411189368e-08	4.98245857868261e-11
86	6.26547330633560e-14	1.08693992796689e-08	4.53721626031848e-11
87	1.10857332032251e-13	1.04959830246299e-08	4.40337912384794e-11
88	1.13529045880108e-13	1.01394776328786e-08	4.60947303401489e-11
89	5.84950513851200e-14	9.79893653936379e-09	4.23365675780945e-11
90	1.52783279524291e-14	9.47347605334385e-09	4.31112585414647e-11
91	1.09763524592131e-13	9.16227053942905e-09	4.28867681411059e-11
92	1.04856247980157e-13	8.86454801615380e-09	4.12524978755205e-11
93	8.68206719323612e-14	8.57958613181725e-09	4.04707611156092e-11
94	4.23715684200737e-14	8.30670848159926e-09	4.02067230362135e-11
95	1.93849187747211e-13	8.04528123373313e-09	3.51506434621134e-11
96	2.40574802860901e-13	7.79471003586184e-09	3.73205362991365e-11
97	1.28890930607113e-13	7.55443717567023e-09	3.76060904133078e-11
98	4.80854922153609e-14	7.32393897252051e-09	3.55471899270564e-11
99	4.26213500169792e-14	7.10272337916127e-09	3.74719257468396e-11
100	4.40884403065375e-14	6.89032777466611e-09	3.52087037873200e-11
101	8.15725313548566e-14	6.68631693161764e-09	3.48111510233251e-11
102	8.74978607328088e-14	6.49028114221218e-09	3.19112446275021e-11
103	5.83093997175917e-14	6.30183448944369e-09	3.21174544599145e-11
104	7.34256825122308e-14	6.12061325085186e-09	3.52644782534737e-11
105	8.49160355261380e-14	5.94627442350771e-09	3.07848388737114e-11
106	8.49519114208932e-14	5.77849435997495e-09	3.02543595083620e-11
107	1.19387163380441e-13	5.61696750594171e-09	2.92207523783373e-11
108	1.29567379975858e-13	5.46140523107591e-09	3.14494710074497e-11
109	9.02888327216997e-14	5.31153474543038e-09	2.91660829648499e-11
110	1.17880646510791e-13	5.16709809441917e-09	2.83588548570514e-11
111	1.10362105463967e-13	5.02785122601338e-09	2.51607278238108e-11
112	3.79112088436668e-14	4.89356312437028e-09	2.69871924356575e-11
113	3.75696452888719e-14	4.76401500462007e-09	2.65729968565424e-11
114	8.08643158866939e-14	4.63899956399594e-09	2.71792861407096e-11
115	7.21611596108906e-14	4.51832028491065e-09	2.55491450076384e-11
116	5.89306747109563e-14	4.40179078596080e-09	2.52412141811496e-11
117	8.80808080959494e-14	4.28923421718233e-09	2.44718150243992e-11
118	8.46890695482763e-14	4.18048269619168e-09	2.30648315097176e-11
119	6.07284359483313e-14	4.07537678212891e-09	2.32339664064555e-11
120	3.80176432457206e-14	3.97376498457543e-09	2.15412902124623e-11
121	6.42108690386734e-14	3.87550330485207e-09	2.35230329193764e-11
122	6.45586334047125e-14	3.78045480731510e-09	2.36302524358651e-11
123	1.09619023856622e-13	3.68848921846117e-09	2.34554269238083e-11
124	8.06917968718153e-14	3.59948255182815e-09	2.45798264072421e-11
125	1.15193985230687e-13	3.51331675683942e-09	2.19128949815386e-11
126	6.70718594592010e-14	3.42987938988579e-09	2.20969654835713e-11
127	5.32902540699704e-14	3.34906330607336e-09	2.21374907777138e-11
128	4.02985161959668e-14	3.27076637018780e-09	1.90197169089014e-11
129	5.39439278749873e-14	3.19489118553789e-09	2.15295557644115e-11
130	1.15148208151762e-13	3.12134483944371e-09	2.14487650484876e-11
131	1.49908418051451e-13	3.05003866422863e-09	1.99825970055646e-11
132	4.35190744419510e-13	2.98088801266085e-09	2.01259550721774e-11
133	3.96817307551225e-13	2.91381204686897e-09	1.85333154662022e-11
134	8.89750118359596e-14	2.84873353982896e-09	1.88197820709739e-11
135	6.33240789260345e-14	2.78557868858628e-09	1.76230311432012e-11
136	7.31793286634457e-14	2.72427693843869e-09	1.71647597850142e-11
137	3.96995741689190e-14	2.66476081736120e-09	1.84294860008329e-11
138	1.75137369381313e-13	2.60696578000689e-09	1.79448785609811e-11
139	1.98163700775295e-13	2.55083006066504e-09	1.92837448069452e-11
140	5.52417408370120e-14	2.49629453460206e-09	1.92262089751609e-11
141	8.10655917068076e-14	2.44330258725136e-09	1.71104388891050e-11
142	8.44436634541483e-14	2.39179999075595e-09	1.63107350699314e-11
143	6.34282438308985e-14	2.34173478740197e-09	1.65861298491760e-11
144	8.67188879441848e-14	2.29305717951341e-09	1.66721209861194e-11
145	8.60969178953438e-14	2.24571942540807e-09	1.59187100747052e-11
146	8.00797022407700e-14	2.19967574104175e-09	1.66745467323055e-11
147	1.09902927349876e-13	2.15488220699326e-09	1.60477550479742e-11
148	1.04969671159329e-13	2.11129668046631e-09	1.57689889095643e-11
149	1.66193965003125e-13	2.06887871200568e-09	1.64894299452926e-11
150	1.64153529761143e-13	2.02758946664560e-09	1.38491840341829e-11
151	7.32860069230108e-14	1.98739164922673e-09	1.43623728266051e-11
152	4.23916760365404e-14	1.94824943363536e-09	1.50818581664617e-11
153	1.16995552915980e-13	1.91012839573463e-09	1.32090103581929e-11
154	1.00198090847954e-13	1.87299544977256e-09	1.36317991306345e-11
155	1.09946066673153e-13	1.83681878806531e-09	1.38992576157901e-11
156	1.37144649823583e-13	1.80156782376713e-09	1.40593829124631e-11
157	1.09636849069155e-13	1.76721313655049e-09	1.41609627186620e-11
158	1.75433570556928e-13	1.73372642103091e-09	1.38149896466055e-11
159	1.31151930784138e-13	1.70108043778149e-09	1.49409517048600e-11
160	1.33597857494977e-13	1.66924896679169e-09	1.42611988619161e-11
161	1.56304154181918e-13	1.63820676323403e-09	1.39119863208775e-11
162	2.28031861748472e-13	1.60792951541090e-09	1.42218773249186e-11
163	1.70016269390512e-13	1.57839380476103e-09	1.34990657450954e-11
164	2.07481395687160e-13	1.54957706781316e-09	1.16179927269503e-11
165	1.31500103744315e-13	1.52145755998067e-09	1.26888790705854e-11
166	1.56925287793059e-13	1.49401432109760e-09	1.23470091885535e-11
167	1.09682036057459e-13	1.46722714260256e-09	1.17029437715606e-11
168	2.03820013209654e-13	1.44107653628213e-09	1.22465678506556e-11
169	1.78483409096072e-13	1.41554370449116e-09	1.13508852575562e-11
170	1.13097209551256e-13	1.39061051177167e-09	1.30976702696936e-11
171	7.33804919910600e-14	1.36625945779712e-09	1.27802699972868e-11
172	1.64726522083945e-13	1.34247365157262e-09	1.28184551605978e-11
173	1.83610612832241e-13	1.31923678682599e-09	9.65335692999623e-12
174	9.90711680148298e-14	1.29653311852819e-09	1.29519317455963e-11
175	8.88904593820075e-14	1.27434744048503e-09	1.15995567682760e-11
176	1.08503949569520e-13	1.25266506394564e-09	1.12286707119368e-11
177	3.70652952130920e-13	1.23147179717601e-09	1.15886070291745e-11
178	4.14972709220376e-13	1.21075392594882e-09	1.09274111015709e-11
179	9.77232236106481e-14	1.19049819490378e-09	1.03218608495932e-11
180	1.05128822195550e-13	1.17069178973480e-09	1.08076037908224e-11
181	4.93589492060864e-14	1.15132232016311e-09	1.00771652920866e-11
182	1.44875292573991e-13	1.13237780365748e-09	1.07814318443780e-11
183	1.53534587200937e-13	1.11384664986484e-09	9.48084562507698e-12
184	5.52347416910348e-14	1.09571764571667e-09	1.08913999378034e-11
185	2.10564271341931e-13	1.07797994117829e-09	9.99289770036476e-12
186	2.12718434329176e-13	1.06062303561001e-09	9.18325931622976e-12
187	1.36514134839365e-13	1.04363676471078e-09	9.90911939313603e-12
188	9.86649401324606e-14	1.02701128801642e-09	9.88142633810915e-12
189	2.15793212670128e-13	1.01073707692620e-09	1.00708590834449e-11
190	2.29895518408631e-13	9.94804903232605e-10	1.03603804435501e-11
191	1.45051125177803e-13	9.79205828130813e-10	1.03073971364127e-11
192	1.78991849804517e-13	9.63931191685258e-10	8.96002655457694e-12
193	1.18731923537460e-13	9.48972602732136e-10	9.25914729224550e-12
194	1.53948275733770e-13	9.34321929197578e-10	9.20808718663561e-12
195	1.48139805983822e-13	9.19971288812380e-10	9.11838482078667e-12
196	2.13347987189723e-13	9.05913040205092e-10	9.37481231465187e-12
197	2.64635933624295e-13	8.92139774356223e-10	8.99754602933704e-12
198	1.74922648906475e-13	8.78644306397153e-10	9.21763090075075e-12
199	8.88046123387018e-14	8.65419667738215e-10	8.21030258466265e-12
200	8.52052494254835e-14	8.52459098511141e-10	9.37778523474801e-12

==> experiments/cubicsqrroot.tex <==
n err bound boundsharp
1	8.53922943307605e-13	2.83931530573942e-08	1.02923516818562e-09
2	1.75358831945095e-12	6.30153629086616e-08	1.66373835729825e-09
3	1.63120898307981e-12	1.05400992660590e-07	2.14235768453289e-09
4	3.00827308832839e-12	1.54419395581518e-07	3.09867946963403e-09
5	2.96903388620827e-12	2.09325028286679e-07	3.81769825231563e-09
6	3.27130703271715e-12	2.69582873546343e-07	4.46057971522681e-09
7	3.32781150992747e-12	3.34785621343787e-07	5.14566027503450e-09
8	4.70854645636959e-12	4.04609995949384e-07	5.70052433972423e-09
9	3.52691424329368e-12	4.78791416021953e-07	6.16038188135961e-09
10	5.81213803643657e-12	5.57108182238288e-07	7.64797254034256e-09
11	6.50717818687278e-12	6.39371041592164e-07	8.03673966286068e-09
12	4.07996605097618e-12	7.25415988663085e-07	9.11421572685753e-09
13	4.69448273523981e-12	8.15099119096846e-07	9.47482472154394e-09
14	4.65165768919213e-12	9.08292840224153e-07	9.89042746698018e-09
15	4.12596787821783e-12	1.00488301115615e-06	1.14326838257904e-08
16	5.96359341802451e-12	1.10476673854837e-06	1.13681552839846e-08
17	5.27926745854793e-12	1.20785064671310e-06	1.24107476836152e-08
18	5.52499250975581e-12	1.31404949847712e-06	1.33455271700598e-08
19	7.18805931016584e-12	1.42328508038225e-06	1.51454328704280e-08
20	4.70082355198481e-12	1.53548529048273e-06	1.61124163498811e-08
21	4.82654977574736e-12	1.65058338374949e-06	1.55282304560021e-08
22	6.79218534693126e-12	1.76851734172448e-06	1.68749939282367e-08
23	4.12264231811556e-12	1.88922934130767e-06	1.76892205082338e-08
24	6.41447291495855e-12	2.01266530349937e-06	1.75150391779704e-08
25	6.47505958694933e-12	2.13877450726448e-06	1.70211573618970e-08
26	4.76385982783807e-12	2.26750925691696e-06	1.77245562516074e-08
27	7.19384646300868e-12	2.39882459385296e-06	2.02777642877460e-08
28	8.27578818323955e-12	2.53267804530843e-06	1.88429597065776e-08
29	6.80468728158092e-12	2.66902940424646e-06	1.87954033083820e-08
30	7.52283422685701e-12	2.80784053558554e-06	2.29014672411003e-08
31	5.79246559572009e-12	2.94907520484881e-06	2.16367421160135e-08
32	7.56439071867934e-12	3.09269892600975e-06	2.38003048286844e-08
33	6.41953759800670e-12	3.23867882585060e-06	2.33717971535190e-08
34	9.43587767415840e-12	3.38698352260501e-06	2.73484895022186e-08
35	6.67678199082152e-12	3.53758301700196e-06	2.72065272612478e-08
36	5.58561062323549e-12	3.69044859413290e-06	2.58252889718201e-08
37	6.73445954676389e-12	3.84555273479497e-06	2.58993941419879e-08
38	3.94949377570534e-12	4.00286903516766e-06	2.60378245814077e-08
39	4.73047912988743e-12	4.16237213384140e-06	2.70427674041473e-08
40	6.92466172383319e-12	4.32403764535489e-06	2.84805425066320e-08
41	7.28412738582908e-12	4.48784209951403e-06	2.96487585439102e-08
42	4.52484825703324e-12	4.65376288586296e-06	2.98789359790978e-08
43	6.99686821382315e-12	4.82177820275364e-06	3.17364439774829e-08
44	6.14070403127201e-12	4.99186701054255e-06	3.41757267865309e-08
45	6.99233700463855e-12	5.16400898848806e-06	3.27895256940455e-08
46	6.69102035127369e-12	5.33818449498385e-06	3.23540098531261e-08
47	5.86440295959160e-12	5.51437453080448e-06	3.33504551465110e-08
48	9.58859677661555e-12	5.69256070507291e-06	3.92927184771381e-08
49	7.18963579228657e-12	5.87272520369955e-06	3.61044994694233e-08
50	6.12046771068074e-12	6.05485076006370e-06	3.80451475346544e-08
51	5.84342881691494e-12	6.23892062774001e-06	3.73819322280119e-08
52	9.48719598719736e-12	6.42491855508621e-06	3.59502088863663e-08
53	6.05378227737560e-12	6.61282876153773e-06	3.90926945509057e-08
54	7.77941669666267e-12	6.80263591545737e-06	4.02935425795234e-08
55	6.89287359311035e-12	6.99432511341627e-06	4.13225619265201e-08
56	8.29952244554891e-12	7.18788186078977e-06	4.04060410310555e-08
57	8.13127038547743e-12	7.38329205355971e-06	4.11119235651031e-08
58	7.36934587872160e-12	7.58054196123019e-06	4.24038515982130e-08
59	7.27942995890433e-12	7.77961821076936e-06	3.99178927536200e-08
60	5.86301292422461e-12	7.98050777150606e-06	4.56538660229396e-08
61	9.12069174898224e-12	8.18319794089363e-06	4.49380256122554e-08
62	8.89433821567408e-12	8.38767633110131e-06	5.15804407628649e-08
63	9.30825877850368e-12	8.59393085634793e-06	4.27432594572643e-08
64	7.74820867928072e-12	8.80194972094391e-06	4.97896000672256e-08
65	8.30444961605404e-12	9.01172140798339e-06	4.40280690727392e-08
66	8.10063757679454e-12	9.22323466864580e-06	4.85266948458438e-08
67	8.93719498585187e-12	9.43647851205513e-06	5.35775247889212e-08
68	1.14784784025308e-11	9.65144219567768e-06	5.37585058198321e-08
69	1.00671130635947e-11	9.86811521620651e-06	5.20347131529543e-08
70	7.63557290566889e-12	1.00864873009079e-05	4.93998653501969e-08
71	6.64340743599699e-12	1.03065483994010e-05	4.75019663846227e-08
72	9.52200175098325e-12	1.05282886758361e-05	5.24865675387932e-08
73	1.23678133434738e-11	1.07516985014638e-05	5.18064023904080e-08
74	9.77138906160123e-12	1.09767684475462e-05	5.06329342392484e-08
75	8.91618440555089e-12	1.12034892786112e-05	5.67670033123823e-08
76	9.88331738349045e-12	1.14318519460156e-05	5.79619081342815e-08
77	1.29536618871914e-11	1.16618475818087e-05	6.02702582933785e-08
78	5.06856090504951e-12	1.18934674928740e-05	6.14619121887253e-08
79	9.79923897166166e-12	1.21267031553232e-05	6.21023280712478e-08
80	7.07773638644989e-12	1.23615462091582e-05	5.82018744915635e-08
81	9.53738944465036e-12	1.25979884531402e-05	6.13564216079171e-08
82	7.74532484012254e-12	1.28360218399064e-05	6.23482182959049e-08
83	9.91345173015265e-12	1.30756384712715e-05	6.04964875497518e-08
84	1.06429386259141e-11	1.33168305937436e-05	6.52598659803253e-08
85	5.93859134398986e-12	1.35595905942204e-05	6.43238384407732e-08
86	7.59815673998309e-12	1.38039109958597e-05	6.42248014361957e-08
87	7.49359824055578e-12	1.40497844541218e-05	6.34936522275303e-08
88	9.74499429262088e-12	1.42972037529681e-05	6.53556502700186e-08
89	1.40285125719589e-11	1.45461618012110e-05	7.04466206706898e-08
90	5.82290857991228e-12	1.47966516290162e-05	6.55812406155077e-08
91	9.38775639736937e-12	1.50486663845181e-05	6.79336075756719e-08
92	7.61364870086560e-12	1.53021993305903e-05	7.42948733150693e-08
93	6.42109890804001e-12	1.55572438417278e-05	6.84713353413440e-08
94	1.07199295891718e-11	1.58137934010425e-05	6.81773646710939e-08
95	8.33802857769850e-12	1.60718415973697e-05	6.43901774725200e-08
96	5.12994606331374e-12	1.63313821225017e-05	7.31264395487944e-08
97	8.70274001469154e-12	1.65924087684906e-05	7.23370910466283e-08
98	7.73027666341815e-12	1.68549154250740e-05	7.30765339825034e-08
99	1.49018967745692e-11	1.71188960771733e-05	7.44809218023825e-08
100	1.00318863233931e-11	1.73843448024994e-05	7.31112116967596e-08
101	7.06482068077814e-12	1.76512557692243e-05	7.81135555584961e-08
102	1.11307802425591e-11	1.79196232337459e-05	8.07052185395100e-08
103	9.45884818671813e-12	1.81894415385243e-05	7.65721309046375e-08
104	1.23232440138111e-11	1.84607051099871e-05	7.79384212787685e-08
105	8.89828530971873e-12	1.87334084565170e-05	7.90663609896128e-08
106	6.90052991460450e-12	1.90075461664965e-05	7.72063946170717e-08
107	9.36893710778543e-12	1.92831129064169e-05	7.70362426013364e-08
108	1.33423113078140e-11	1.95601034190530e-05	7.88309541548304e-08
109	7.66505099178671e-12	1.98385125217043e-05	8.07872972785622e-08
110	1.41399661884032e-11	2.01183351044711e-05	8.99865685816764e-08
111	9.89095493667729e-12	2.03995661286070e-05	8.32856713061965e-08
112	1.11538064809722e-11	2.06822006249197e-05	8.77810208740336e-08
113	1.42311347138979e-11	2.09662336922017e-05	9.53465658191043e-08
114	1.12644453092419e-11	2.12516604957369e-05	8.74700526444383e-08
115	9.05348036848094e-12	2.15384762658388e-05	9.44855348982330e-08
116	7.57896291026093e-12	2.18266762964330e-05	9.30784750734867e-08
117	8.26828192719907e-12	2.21162559436946e-05	8.68066756915391e-08
118	1.07187636660588e-11	2.24072106246906e-05	8.43306853311036e-08
119	1.32590188450355e-11	2.26995358161197e-05	8.63601398799083e-08
120	1.00137946958897e-11	2.29932270530446e-05	8.70935570280024e-08
121	1.37948466116456e-11	2.32882799276650e-05	8.93729766274029e-08
122	8.85307952468260e-12	2.35846900881532e-05	9.24156342525459e-08
123	1.56739801010136e-11	2.38824532374945e-05	9.52044090358235e-08
124	8.62059774524641e-12	2.41815651323649e-05	9.07951561416564e-08
125	1.18813157522135e-11	2.44820215820785e-05	9.85458498276929e-08
126	7.43385213333605e-12	2.47838184474893e-05	9.02153563046928e-08
127	7.78035327087434e-12	2.50869516399918e-05	9.28514744664403e-08
128	1.89618031900945e-11	2.53914171205419e-05	1.01221058439801e-07
129	8.90966292445275e-12	2.56972108986382e-05	9.77638768539646e-08
130	1.44947413304062e-11	2.60043290314240e-05	9.98202447476480e-08
131	1.41892526966127e-11	2.63127676227608e-05	1.06783423102175e-07
132	9.35076926567758e-12	2.66225228223081e-05	9.61314556622059e-08
133	1.54459458295171e-11	2.69335908246974e-05	9.39410973189410e-08
134	1.04095933995069e-11	2.72459678686433e-05	1.08097910349234e-07
135	1.38535014386635e-11	2.75596502361483e-05	1.04795572404035e-07
136	9.75190420875858e-12	2.78746342516970e-05	1.12115980777526e-07
137	1.31038429152925e-11	2.81909162814554e-05	1.04840394088842e-07
138	8.17978159951091e-12	2.85084927325202e-05	1.10349710925223e-07
139	1.51669304060254e-11	2.88273600521845e-05	1.14160180340687e-07
140	1.12002497333450e-11	2.91475147272072e-05	1.12686106652829e-07
141	1.13623371982687e-11	2.94689532830890e-05	1.07123089177197e-07
142	1.01876718815621e-11	2.97916722834130e-05	1.18426350241485e-07
143	1.03144663902389e-11	3.01156683291603e-05	1.12061360894163e-07
144	1.13390564230173e-11	3.04409380580419e-05	9.71660335495517e-08
145	1.06249771802337e-11	3.07674781438847e-05	9.91932125794577e-08
146	1.00010737633141e-11	3.10952852959871e-05	1.20258479547496e-07
147	1.44555655917612e-11	3.14243562585175e-05	1.23427472677771e-07
148	1.03623477257228e-11	3.17546878099223e-05	1.18811909085573e-07
149	9.90526817963963e-12	3.20862767623413e-05	1.06220330332466e-07
150	1.78790418741075e-11	3.24191199610481e-05	1.15528586617925e-07
151	1.45792184074381e-11	3.27532142838869e-05	1.22323330912444e-07
152	1.57177057877277e-11	3.30885566407269e-05	1.22878241457119e-07
153	8.51992756789705e-12	3.34251439729597e-05	1.14050743463986e-07
154	1.80496297273273e-11	3.37629732529661e-05	1.20779510883238e-07
155	1.46227109242470e-11	3.41020414835964e-05	1.11896753507069e-07
156	1.57540874302549e-11	3.44423456977091e-05	1.28523021255480e-07
157	1.67708943129492e-11	3.47838829576633e-05	1.33622338317412e-07
158	1.24414155229514e-11	3.51266503548716e-05	1.10458132378707e-07
159	1.60582531806384e-11	3.54706450093045e-05	1.33587839578224e-07
160	1.48199820525670e-11	3.58158640690867e-05	1.29641884665872e-07
161	8.91766763200700e-12	3.61623047100019e-05	1.29538694794231e-07
162	9.94657302319134e-12	3.65099641351145e-05	1.26185039988758e-07
163	1.57432321089693e-11	3.68588395743081e-05	1.22274734867106e-07
164	1.56351367295716e-11	3.72089282838971e-05	1.43470660118084e-07
165	1.43125770767067e-11	3.75602275462120e-05	1.37400944196166e-07
166	1.66132561063304e-11	3.79127346692028e-05	1.37953804793621e-07
167	1.66680625909662e-11	3.82664469860529e-05	1.23752754158906e-07
168	1.22640246407344e-11	3.86213618548106e-05	1.30606795874617e-07
169	1.44232392433106e-11	3.89774766579987e-05	1.28835981869659e-07
170	1.33963840106356e-11	3.93347888022811e-05	1.32311142603801e-07
171	9.41587025007437e-12	3.96932957180648e-05	1.20596415423410e-07
172	1.47127759398378e-11	4.00529948591822e-05	1.32994162906504e-07
173	1.46225142980301e-11	4.04138837025563e-05	1.34864130412829e-07
174	1.45613706721367e-11	4.07759597478401e-05	1.33082896531385e-07
175	2.04980057103136e-11	4.11392205170915e-05	1.28220056177856e-07
176	1.08347177441449e-11	4.15036635544815e-05	1.41600362589087e-07
177	2.44892475560824e-11	4.18692864259403e-05	1.48941339510375e-07
178	1.36712335147266e-11	4.22360867188893e-05	1.16855322445708e-07
179	1.63585104822358e-11	4.26040620418871e-05	1.31780657850601e-07
180	1.21209265529291e-11	4.29732100243967e-05	1.35702155718528e-07
181	1.28952209515625e-11	4.33435283164203e-05	1.44909579561655e-07
182	1.42002234377678e-11	4.37150145882985e-05	1.51694916931330e-07
183	1.12227298014807e-11	4.40876665303514e-05	1.38859336148890e-07
184	2.32727787008797e-11	4.44614818526535e-05	1.34573436077610e-07
185	1.04999074601736e-11	4.48364582847604e-05	1.33367520310430e-07
186	1.30027329672943e-11	4.52125935753955e-05	1.36847731425775e-07
187	2.82239755525900e-11	4.55898854922930e-05	1.56368385915784e-07
188	1.24768050364599e-11	4.59683318218108e-05	1.50062377540369e-07
189	1.30013017763175e-11	4.63479303688123e-05	1.45761671711185e-07
190	1.08077474301167e-11	4.67286789563101e-05	1.29310654274274e-07
191	1.48191783101876e-11	4.71105754253185e-05	1.48065928690739e-07
192	2.61257304985525e-11	4.74936176345318e-05	1.39046920293341e-07
193	1.34339762912138e-11	4.78778034601737e-05	1.66058164515852e-07
194	1.12124705227033e-11	4.82631307957149e-05	1.56471783670259e-07
195	1.63455763408259e-11	4.86495975516567e-05	1.41833911405214e-07
196	1.47925290897693e-11	4.90372016553472e-05	1.55307083503343e-07
197	3.84634523302576e-11	4.94259410507080e-05	1.62368389106226e-07
198	1.54519341165455e-11	4.98158136980823e-05	1.62074388401984e-07
199	2.65958637274431e-11	5.02068175739935e-05	1.50061697420349e-07
200	1.18780077362693e-11	5.02068175739935e-05	1.67003477109072e-07

==> experiments/jordan.tex <==
n real imag
1	-0.656231741478211	0.531402499691787
2	-0.656231741478211	-0.531402499691787
3	-0.690741096543285	0.489199379606050
4	-0.690741096543285	-0.489199379606050
5	-0.722928122825179	0.444375728668951
6	-0.722928122825179	-0.444375728668951
7	-0.752305774160921	0.396176330846032
8	-0.752305774160921	-0.396176330846032
9	-0.776994326723648	0.344858971160430
10	-0.776994326723648	-0.344858971160430
11	-0.619333488599878	0.570721885557701
12	-0.619333488599878	-0.570721885557701
13	-0.795997782094739	0.292979145954847
14	-0.795997782094739	-0.292979145954847
15	-0.581250836671729	0.607195354509133
16	-0.581250836671729	-0.607195354509133
17	-0.851289638703800	0.0280729613875431
18	-0.851289638703800	-0.0280729613875431
19	-0.541920852473072	0.642588502248715
20	-0.541920852473072	-0.642588502248715
21	-0.811951064789207	0.242685253317069
22	-0.811951064789207	-0.242685253317069
23	-0.499538817408402	0.677211161527784
24	-0.499538817408402	-0.677211161527784
25	-0.846783723689446	0.0835300578212094
26	-0.846783723689446	-0.0835300578212094
27	-0.453034051404882	0.709915162107499
28	-0.453034051404882	-0.709915162107499
29	-0.402400334204730	0.740069183215739
30	-0.402400334204730	-0.740069183215739
31	-0.826888725566270	0.191389766659376
32	-0.826888725566270	-0.191389766659376
33	-0.347349028417533	0.767573458329300
34	-0.347349028417533	-0.767573458329300
35	-0.288901780047628	0.791122248667596
36	-0.288901780047628	-0.791122248667596
37	-0.287959889401400	0.653403262026084
38	-0.287959889401400	-0.653403262026084
39	-0.229223898786470	0.808567855573007
40	-0.229223898786470	-0.808567855573007
41	0.288559994747971	0.796192600749964
42	0.288559994747971	-0.796192600749964
43	0.341035248117080	0.774435091733476
44	0.341035248117080	-0.774435091733476
45	0.390124224476670	0.748686347753116
46	0.390124224476670	-0.748686347753116
47	0.234213967289327	0.813031122986604
48	0.234213967289327	-0.813031122986604
49	0.435744348238741	0.720837054057983
50	0.435744348238741	-0.720837054057983
51	0.179015329526647	0.825499688892064
52	0.179015329526647	-0.825499688892064
53	0.479110815173490	0.691863200496914
54	0.479110815173490	-0.691863200496914
55	0.521572683822514	0.661388150794890
56	0.521572683822514	-0.661388150794890
57	0.562953109267616	0.628051259891888
58	0.562953109267616	-0.628051259891888
59	0.122429060881885	0.833725811972092
60	0.122429060881885	-0.833725811972092
61	0.602363555433597	0.592318892054741
62	0.602363555433597	-0.592318892054741
63	-0.169847669600893	0.819535614487963
64	-0.169847669600893	-0.819535614487963
65	0.640710743345408	0.554147414771460
66	0.640710743345408	-0.554147414771460
67	0.677371986259180	0.512058758971110
68	0.677371986259180	-0.512058758971110
69	0.0648409613658542	0.835950956929346
70	0.0648409613658542	-0.835950956929346
71	0.710378256762231	0.466266754907730
72	0.710378256762231	-0.466266754907730
73	-0.109542932035438	0.824791872206828
74	-0.109542932035438	-0.824791872206828
75	0.739303647949573	0.418462267086674
76	0.739303647949573	-0.418462267086674
77	0.764579101786262	0.368896171907034
78	0.764579101786262	-0.368896171907034
79	0.832047635513370	0.162048905939247
80	0.832047635513370	-0.162048905939247
81	0.840549681976116	0.107993137086400
82	0.840549681976116	-0.107993137086400
83	0.820070134324406	0.215409095097710
84	0.820070134324406	-0.215409095097710
85	0.845108826777746	0.0537172057616339
86	0.845108826777746	-0.0537172057616339
87	0.00889251823871104	0.832256501323933
88	0.00889251823871104	-0.832256501323933
89	0.804294874015953	0.267832145324688
90	0.804294874015953	-0.267832145324688
91	-0.0620113124438114	0.765352631028257
92	-0.0620113124438114	-0.765352631028257
93	-0.838689725584223	0.137963343730069
94	-0.838689725584223	-0.137963343730069
95	0.846413398188992	0
96	-0.0475270761529973	0.827209400472414
97	-0.0475270761529973	-0.827209400472414
98	0.785713013194973	0.318480086839835
99	0.785713013194973	-0.318480086839835
100	0.192906544455946	0

==> experiments/linearequi.tex <==
n err bound boundsharp
1	5.79227939839670e-06	0.00100200400801603	5.80387000811646e-06
2	5.49387981763653e-06	0.00100200400801603	5.50481358731819e-06
3	5.21588733631179e-06	0.00100200400801603	5.22633900808381e-06
4	5.97633511360369e-06	0.00100200400801603	5.98831936558224e-06
5	5.17169892513277e-06	0.00100200400801603	5.18206333593743e-06
6	5.36518924226002e-06	0.00100200400801603	5.37594710045049e-06
7	5.14560622189715e-06	0.00100200400801603	5.15590529957585e-06
8	5.58732603494087e-06	0.00100200400801603	5.59852748858686e-06
9	5.29216432024713e-06	0.00100200400801603	5.30272861947737e-06
10	5.72022029358028e-06	0.00100200400801603	5.73173443180814e-06
11	5.71846172796991e-06	0.00100200400801603	5.72992581118820e-06
12	5.23760803252611e-06	0.00100200400801603	5.24810702136740e-06
13	5.26289501360781e-06	0.00100200400801603	5.27349278685663e-06
14	5.77717728197166e-06	0.00100200400801603	5.78877906240643e-06
15	5.63497156243338e-06	0.00100200400801603	5.64627085251628e-06
16	5.44739832754325e-06	0.00100200400801603	5.45831041053019e-06
17	5.28394350462955e-06	0.00100200400801603	5.29453305184494e-06
18	5.44209288834824e-06	0.00100200400801603	5.45301419711598e-06
19	5.75952876597556e-06	0.00100200400801603	5.77105056308613e-06
20	5.06896686171622e-06	0.00100200400801603	5.07909413988125e-06
21	5.46381703900691e-06	0.00100200400801603	5.47478656797974e-06
22	5.63752931259994e-06	0.00100200400801603	5.64880481404381e-06
23	5.58423158951426e-06	0.00100200400801603	5.59543371910866e-06
24	5.57815076870153e-06	0.00100200400801603	5.58933781379369e-06
25	5.82384655018284e-06	0.00100200400801603	5.83552052108578e-06
26	5.48719284611451e-06	0.00100200400801603	5.49818980112494e-06
27	5.21846684264736e-06	0.00100200400801603	5.22886414148254e-06
28	5.22616172968732e-06	0.00100200400801603	5.23661648477537e-06
29	5.23232097493772e-06	0.00100200400801603	5.24278540023950e-06
30	5.52957337758104e-06	0.00100200400801603	5.54064794690055e-06
31	5.49602743495250e-06	0.00100200400801603	5.50704541713391e-06
32	5.55613742192176e-06	0.00100200400801603	5.56726351472478e-06
33	5.63059118910355e-06	0.00100200400801603	5.64188559763638e-06
34	4.97741559104111e-06	0.00100200400801603	4.98739684244459e-06
35	5.51237642848684e-06	0.00100200400801603	5.52342490370085e-06
36	5.23787325905230e-06	0.00100200400801603	5.24837533910233e-06
37	5.91029719006563e-06	0.00100200400801603	5.92213852419289e-06
38	5.69552426811505e-06	0.00100200400801603	5.70697668877472e-06
39	5.55279307107219e-06	0.00100200400801603	5.56390068339642e-06
40	5.50557225511224e-06	0.00100200400801603	5.51659459813836e-06
41	5.55910544403306e-06	0.00100200400801603	5.57027754851359e-06
42	5.15046379889837e-06	0.00100200400801603	5.16076466083396e-06
43	6.04463867601248e-06	0.00100200400801603	6.05676635682309e-06
44	5.04311844537350e-06	0.00100200400801603	5.05325581054795e-06
45	5.49782406842443e-06	0.00100200400801603	5.50883128315970e-06
46	5.57004808457792e-06	0.00100200400801603	5.58121370036494e-06
47	5.63441771979142e-06	0.00100200400801603	5.64577904812417e-06
48	5.38981737258620e-06	0.00100200400801603	5.40062922115592e-06
49	4.76188536971041e-06	0.00100200400801603	4.77144323882229e-06
50	5.67797291910201e-06	0.00100200400801603	5.68934653689488e-06
51	5.43772470104397e-06	0.00100200400801603	5.44861690249849e-06
52	5.36673429660240e-06	0.00100200400801603	5.37754190753022e-06
53	5.63702335620097e-06	0.00100200400801603	5.64833907571547e-06
54	5.57955630036746e-06	0.00100200400801603	5.59075111003376e-06
55	5.85888144646970e-06	0.00100200400801603	5.87061758588136e-06
56	5.23473762382143e-06	0.00100200400801603	5.24526329478028e-06
57	5.34100278361814e-06	0.00100200400801603	5.35169673693094e-06
58	6.02231401947265e-06	0.00100200400801603	6.03437500009230e-06
59	5.67817763312418e-06	0.00100200400801603	5.68956403204162e-06
60	5.70891832914473e-06	0.00100200400801603	5.72036433705863e-06
61	5.00944919529178e-06	0.00100200400801603	5.01948301972117e-06
62	5.10076293515731e-06	0.00100200400801603	5.11100260227355e-06
63	5.13252730842650e-06	0.00100200400801603	5.14277779131719e-06
64	5.27816826421479e-06	0.00100200400801603	5.28876032251398e-06
65	5.30828663678003e-06	0.00100200400801603	5.31890204560220e-06
66	5.57357617080256e-06	0.00100200400801603	5.58473739491821e-06
67	5.56692636327676e-06	0.00100200400801603	5.57807952660404e-06
68	5.72801950000628e-06	0.00100200400801603	5.73949027954675e-06
69	5.34966549709621e-06	0.00100200400801603	5.36036301139718e-06
70	4.92178630959964e-06	0.00100200400801603	4.93166274341928e-06
71	5.77258198765576e-06	0.00100200400801603	5.78415462223313e-06
72	5.96473878175043e-06	0.00100200400801603	5.97672674331368e-06
73	5.25313292805334e-06	0.00100200400801603	5.26364545331594e-06
74	5.62863083908599e-06	0.00100200400801603	5.63992366219770e-06
75	5.70229688162154e-06	0.00100200400801603	5.71368992218041e-06
76	5.67628362993543e-06	0.00100200400801603	5.68766571487468e-06
77	4.81780888759158e-06	0.00100200400801603	4.82746630823115e-06
78	6.10553193803085e-06	0.00100200400801603	6.11777711353249e-06
79	5.50869892025041e-06	0.00100200400801603	5.51980165160587e-06
80	5.78381084104136e-06	0.00100200400801603	5.79536431727561e-06
81	5.25065525909111e-06	0.00100200400801603	5.26118595213535e-06
82	5.37191810464266e-06	0.00100200400801603	5.38268433831092e-06
83	5.29588958252223e-06	0.00100200400801603	5.30648445387367e-06
84	5.39091919223849e-06	0.00100200400801603	5.40172348420059e-06
85	5.75319603521210e-06	0.00100200400801603	5.76469992732326e-06
86	5.29003424041637e-06	0.00100200400801603	5.30064546109262e-06
87	5.24123378314590e-06	0.00100200400801603	5.25174027273309e-06
88	5.19170938502820e-06	0.00100200400801603	5.20208969915893e-06
89	5.44669971537362e-06	0.00100200400801603	5.45762038400579e-06
90	5.32434700441341e-06	0.00100200400801603	5.33499885808952e-06
91	5.34124977909289e-06	0.00100200400801603	5.35197998723922e-06
92	5.60770866605846e-06	0.00100200400801603	5.61895498553876e-06
93	5.97498014081318e-06	0.00100200400801603	5.98694850982591e-06
94	5.39912346332654e-06	0.00100200400801603	5.40994046554721e-06
95	5.70482195785790e-06	0.00100200400801603	5.71621283324931e-06
96	5.36063225181571e-06	0.00100200400801603	5.37137808085872e-06
97	5.71955204711244e-06	0.00100200400801603	5.73100769344880e-06
98	5.50310610852257e-06	0.00100200400801603	5.51412435946458e-06
99	5.57903392880355e-06	0.00100200400801603	5.59023014054369e-06
100	5.64642690915396e-06	0.00100200400801603	5.65773214148177e-06
101	5.66265315693879e-06	0.00100200400801603	5.67401705949606e-06
102	5.45431829648299e-06	0.00100200400801603	5.46523888312981e-06
103	5.16888256399177e-06	0.00100200400801603	5.17924865256459e-06
104	5.50318643133091e-06	0.00100200400801603	5.51423627235058e-06
105	5.10491157756053e-06	0.00100200400801603	5.11513931461550e-06
106	5.63733411516345e-06	0.00100200400801603	5.64860059675850e-06
107	5.46196059603354e-06	0.00100200400801603	5.47291743418717e-06
108	5.66043854633280e-06	0.00100200400801603	5.67176748242832e-06
109	5.16710448735682e-06	0.00100200400801603	5.17745356240513e-06
110	5.09875701277118e-06	0.00100200400801603	5.10896329603643e-06
111	5.77169045073805e-06	0.00100200400801603	5.78326942922259e-06
112	5.93602928857237e-06	0.00100200400801603	5.94794989183936e-06
113	5.12426107913376e-06	0.00100200400801603	5.13456134389399e-06
114	5.55410789778241e-06	0.00100200400801603	5.56525023565753e-06
115	6.02287713389120e-06	0.00100200400801603	6.03496222421483e-06
116	6.07580507658641e-06	0.00100200400801603	6.08796457840102e-06
117	6.10770313977209e-06	0.00100200400801603	6.11993896701690e-06
118	5.63206455915986e-06	0.00100200400801603	5.64335592844597e-06
119	5.04191465071124e-06	0.00100200400801603	5.05201276798200e-06
120	5.71228174934462e-06	0.00100200400801603	5.72374958571184e-06
121	5.89463116006625e-06	0.00100200400801603	5.90642662867758e-06
122	5.61072230701529e-06	0.00100200400801603	5.62194399381582e-06
123	6.15117411358795e-06	0.00100200400801603	6.16352407795028e-06
124	5.52738128688450e-06	0.00100200400801603	5.53845381093603e-06
125	5.42274049761356e-06	0.00100200400801603	5.43360001092768e-06
126	5.73052930198938e-06	0.00100200400801603	5.74199626274139e-06
127	5.60424154038628e-06	0.00100200400801603	5.61545943084450e-06
128	5.55635350257939e-06	0.00100200400801603	5.56748593284843e-06
129	5.55116408449533e-06	0.00100200400801603	5.56228042671311e-06
130	5.71984198520486e-06	0.00100200400801603	5.73130414829704e-06
131	5.69618451454426e-06	0.00100200400801603	5.70758426337853e-06
132	5.46281875800496e-06	0.00100200400801603	5.47376514229875e-06
133	5.64716454887193e-06	0.00100200400801603	5.65847893121425e-06
134	5.09832826884632e-06	0.00100200400801603	5.10855930984762e-06
135	5.66165284456999e-06	0.00100200400801603	5.67300994777673e-06
136	5.29915879836660e-06	0.00100200400801603	5.30978231006890e-06
137	5.49485724021640e-06	0.00100200400801603	5.50587893963985e-06
138	5.51572359802450e-06	0.00100200400801603	5.52679473910389e-06
139	5.53077603699598e-06	0.00100200400801603	5.54183895076120e-06
140	5.92161198378492e-06	0.00100200400801603	5.93349380130304e-06
141	5.46832290612660e-06	0.00100200400801603	5.47924879101832e-06
142	5.74118555371680e-06	0.00100200400801603	5.75271959100689e-06
143	5.44545624015256e-06	0.00100200400801603	5.45635828892859e-06
144	5.23886596054758e-06	0.00100200400801603	5.24936287882144e-06
145	5.61282721683553e-06	0.00100200400801603	5.62408412396303e-06
146	5.39243298624327e-06	0.00100200400801603	5.40322746500255e-06
147	5.65223317601763e-06	0.00100200400801603	5.66355205239872e-06
148	5.82756914248325e-06	0.00100200400801603	5.83927531743222e-06
149	5.91601440616424e-06	0.00100200400801603	5.92782190608533e-06
150	5.41149996436295e-06	0.00100200400801603	5.42233814979764e-06
151	5.96199639973910e-06	0.00100200400801603	5.97394129646620e-06
152	5.57858021997246e-06	0.00100200400801603	5.58974700833332e-06
153	5.19554045623072e-06	0.00100200400801603	5.20594078187395e-06
154	5.78621902653417e-06	0.00100200400801603	5.79782969220364e-06
155	5.52974550623165e-06	0.00100200400801603	5.54083774711738e-06
156	5.33647480336155e-06	0.00100200400801603	5.34717812588230e-06
157	5.60439473111164e-06	0.00100200400801603	5.61566401145600e-06
158	5.82806189336902e-06	0.00100200400801603	5.83977348421246e-06
159	5.80239756087023e-06	0.00100200400801603	5.81403642017373e-06
160	5.34484958518766e-06	0.00100200400801603	5.35556778071436e-06
161	5.64851483934483e-06	0.00100200400801603	5.65982712875184e-06
162	5.22111432645759e-06	0.00100200400801603	5.23161724002375e-06
163	5.75385432328784e-06	0.00100200400801603	5.76539518126697e-06
164	6.07447281561533e-06	0.00100200400801603	6.08659008113358e-06
165	5.34755522259028e-06	0.00100200400801603	5.35831935206404e-06
166	5.33531624931510e-06	0.00100200400801603	5.34600892971540e-06
167	5.55187559025600e-06	0.00100200400801603	5.56301615383394e-06
168	5.55505738400583e-06	0.00100200400801603	5.56618670381905e-06
169	5.59853307784504e-06	0.00100200400801603	5.60974619080352e-06
170	4.86594084708686e-06	0.00100200400801603	4.87569452388831e-06
171	5.33827971225293e-06	0.00100200400801603	5.34896216185841e-06
172	5.58455974118098e-06	0.00100200400801603	5.59576255124457e-06
173	5.64246222158079e-06	0.00100200400801603	5.65378971798963e-06
174	6.04739348646462e-06	0.00100200400801603	6.05953544973084e-06
175	5.33912809840950e-06	0.00100200400801603	5.34983503729255e-06
176	5.32735987117055e-06	0.00100200400801603	5.33803909238499e-06
177	5.30586216821437e-06	0.00100200400801603	5.31655350559226e-06
178	5.67103614946921e-06	0.00100200400801603	5.68238977098513e-06
179	5.57261564430030e-06	0.00100200400801603	5.58379693464216e-06
180	5.92561337945514e-06	0.00100200400801603	5.93753982019998e-06
181	5.39191738244560e-06	0.00100200400801603	5.40273174620030e-06
182	5.36817879279631e-06	0.00100200400801603	5.37894203245275e-06
183	5.50332379881990e-06	0.00100200400801603	5.51438488171771e-06
184	5.64435074950785e-06	0.00100200400801603	5.65563318048574e-06
185	5.35354306837786e-06	0.00100200400801603	5.36423878844671e-06
186	5.63081399320360e-06	0.00100200400801603	5.64212614607945e-06
187	5.31656958822822e-06	0.00100200400801603	5.32718800540447e-06
188	5.82810912163468e-06	0.00100200400801603	5.83977535921481e-06
189	5.05053118582589e-06	0.00100200400801603	5.06065860441718e-06
190	5.00940110564206e-06	0.00100200400801603	5.01948560968196e-06
191	5.56552032929324e-06	0.00100200400801603	5.57666027315229e-06
192	5.93577120108892e-06	0.00100200400801603	5.94767028477904e-06
193	5.76119495084591e-06	0.00100200400801603	5.77270011997950e-06
194	5.96187500174564e-06	0.00100200400801603	5.97378703850783e-06
195	5.29972743975637e-06	0.00100200400801603	5.31038148940723e-06
196	5.49142619029035e-06	0.00100200400801603	5.50240100479387e-06
197	5.78447436272355e-06	0.00100200400801603	5.79603404112873e-06
198	5.43497624631656e-06	0.00100200400801603	5.44588694928698e-06
199	5.75536648851089e-06	0.00100200400801603	5.76693091894094e-06
200	5.79397374792172e-06	0.00100200400801603	5.80556722717489e-06

==> experiments/linearpow2.tex <==
n err bound boundsharp
1	6.73825587933936e-06	0.125000000000000	8.42268888066862e-06
2	7.97437275179622e-06	0.125000000000000	9.96852470579208e-06
3	7.65369732206523e-06	0.0681818181818182	8.69748948097964e-06
4	7.59330639133989e-06	0.0468750000000000	8.30526898323977e-06
5	7.88532289213216e-06	0.0357142857142857	8.44872009776504e-06
6	6.82493423373751e-06	0.0288461538461538	7.21907594052011e-06
7	7.20909901245343e-06	0.0241935483870968	7.55883984079017e-06
8	7.54719074967856e-06	0.0208333333333333	7.86120051580331e-06
9	7.52538695863793e-06	0.0182926829268293	7.80130151893083e-06
10	7.42631569751858e-06	0.0163043478260870	7.66900643740150e-06
11	7.75714249835228e-06	0.0147058823529412	7.98596018410693e-06
12	7.38535271879173e-06	0.0133928571428571	7.58368486382512e-06
13	7.98841121120315e-06	0.0122950819672131	8.18503763062017e-06
14	7.56332491209556e-06	0.0113636363636364	7.73495391952366e-06
15	7.01699101362723e-06	0.0105633802816901	7.16518108215336e-06
16	8.16678891739187e-06	0.00986842105263158	8.32750855864192e-06
17	7.73000643861586e-06	0.00925925925925926	7.87309988843725e-06
18	7.24137628752058e-06	0.00872093023255814	7.36721484333504e-06
19	7.55250346611592e-06	0.00824175824175824	7.67743037018096e-06
20	7.53152931696887e-06	0.00781250000000000	7.64951837405786e-06
21	7.44887932778546e-06	0.00742574257425743	7.56004196098822e-06
22	7.26714261878760e-06	0.00707547169811321	7.37007920862963e-06
23	7.09851432250272e-06	0.00675675675675676	7.19416584781246e-06
24	8.03399591383121e-06	0.00646551724137931	8.13782789259843e-06
25	7.83959595949578e-06	0.00619834710743802	7.93653993918336e-06
26	7.82231550555056e-06	0.00595238095238095	7.91547481660816e-06
27	8.19398382332703e-06	0.00572519083969466	8.28763469212489e-06
28	7.36479962685842e-06	0.00551470588235294	7.44589978848474e-06
29	7.40855326287728e-06	0.00531914893617021	7.48755710501377e-06
30	7.37658157738840e-06	0.00513698630136986	7.45238912215416e-06
31	7.57109876094471e-06	0.00496688741721854	7.64612231991195e-06
32	7.95668679695943e-06	0.00480769230769231	8.03333759851220e-06
33	7.84022849209575e-06	0.00465838509316770	7.91349796814692e-06
34	7.23636155125801e-06	0.00451807228915663	7.30196884904829e-06
35	8.07149810951337e-06	0.00438596491228070	8.14232085023731e-06
36	7.36841898604692e-06	0.00426136363636364	7.43121195486065e-06
37	7.25623457679828e-06	0.00414364640883978	7.31645800988925e-06
38	7.63555214800456e-06	0.00403225806451613	7.69706002187000e-06
39	8.01345724848942e-06	0.00392670157068063	8.07635729829479e-06
40	7.71003325473108e-06	0.00382653061224490	7.76895117130257e-06
41	7.06083184095267e-06	0.00373134328358209	7.11350849921787e-06
42	7.18776807550697e-06	0.00364077669902913	7.23987861184471e-06
43	7.65214729508989e-06	0.00355450236966825	7.70665786275996e-06
44	7.48426729520187e-06	0.00347222222222222	7.53621677176115e-06
45	7.91045310220295e-06	0.00339366515837104	7.96423844756254e-06
46	6.98706741470721e-06	0.00331858407079646	7.03318253016731e-06
47	7.64710280298823e-06	0.00324675324675325	7.69671650974853e-06
48	7.60366944182427e-06	0.00317796610169492	7.65205945480046e-06
49	8.07703621420515e-06	0.00311203319502075	8.12738181050761e-06
50	7.57251050631881e-06	0.00304878048780488	7.61870623321672e-06
51	7.22333685039299e-06	0.00298804780876494	7.26644640048352e-06
52	7.67077662474710e-06	0.00292968750000000	7.71562956326630e-06
53	7.57301906605487e-06	0.00287356321839080	7.61662213056264e-06
54	7.79202876043089e-06	0.00281954887218045	7.83590488587312e-06
55	7.73691190700429e-06	0.00276752767527675	7.77976011562169e-06
56	7.12634321257292e-06	0.00271739130434783	7.16500634316930e-06
57	7.67078910586248e-06	0.00266903914590747	7.71175464396910e-06
58	7.95277255184160e-06	0.00262237762237762	7.99455788246265e-06
59	7.93591049402437e-06	0.00257731958762887	7.97684939213012e-06
60	7.28945051752284e-06	0.00253378378378378	7.32642530103056e-06
61	6.95113785904156e-06	0.00249169435215947	6.98580528449757e-06
62	8.06652329609447e-06	0.00245098039215686	8.10606292889854e-06
63	6.90217805883470e-06	0.00241157556270097	6.93544383387514e-06
64	7.62386041386930e-06	0.00237341772151899	7.66002754241101e-06
65	7.51322518282856e-06	0.00233644859813084	7.54833866957306e-06
66	8.07623944017530e-06	0.00230061349693252	8.11342139312307e-06
67	7.57805328617220e-06	0.00226586102719033	7.61244967636121e-06
68	7.81740556998767e-06	0.00223214285714286	7.85227240292631e-06
69	7.02749168825942e-06	0.00219941348973607	7.05852813044764e-06
70	7.79306269258521e-06	0.00216763005780347	7.82677791409976e-06
71	7.57953332247496e-06	0.00213675213675214	7.61191401356143e-06
72	7.21458843664392e-06	0.00210674157303371	7.24502918611062e-06
73	7.46877747951464e-06	0.00207756232686981	7.49980906721916e-06
74	7.20186728236441e-06	0.00204918032786885	7.23139591048987e-06
75	7.60767995278882e-06	0.00202156334231806	7.63841804138858e-06
76	7.04474712211534e-06	0.00199468085106383	7.07260644107828e-06
77	7.81932914499203e-06	0.00196850393700787	7.85013401961354e-06
78	7.28860496779458e-06	0.00194300518134715	7.31694426014931e-06
79	7.62026209342968e-06	0.00191815856777494	7.64946144398750e-06
80	7.54842861866248e-06	0.00189393939393939	7.57698231434296e-06
81	8.53794452188564e-06	0.00187032418952618	8.56982293609447e-06
82	8.07582589858057e-06	0.00184729064039409	8.10562570095463e-06
83	7.32126606817237e-06	0.00182481751824818	7.34795718846778e-06
84	8.05814755073632e-06	0.00180288461538462	8.08717828274535e-06
85	7.85435132582878e-06	0.00178147268408551	7.88235318063027e-06
86	7.32336678858775e-06	0.00176056338028169	7.34912444635001e-06
87	7.27515688700521e-06	0.00174013921113689	7.30040498058030e-06
88	7.79322804253759e-06	0.00172018348623853	7.82006695065134e-06
89	7.32289003520370e-06	0.00170068027210884	7.34783463283282e-06
90	7.62693769236051e-06	0.00168161434977578	7.65257763802885e-06
91	7.75819368559685e-06	0.00166297117516630	7.78403769107037e-06
92	7.62883631615494e-06	0.00164473684210526	7.65402849204450e-06
93	7.64932609747982e-06	0.00162689804772234	7.67423990355999e-06
94	7.76511869127031e-06	0.00160944206008584	7.79013628515415e-06
95	6.93507363579226e-06	0.00159235668789809	6.95716663901449e-06
96	7.52033242923232e-06	0.00157563025210084	7.54400943037072e-06
97	7.73784677587193e-06	0.00155925155925156	7.76197534650924e-06
98	7.46705920800877e-06	0.00154320987654321	7.49006440176711e-06
99	8.03408434989307e-06	0.00152749490835031	8.05862381636735e-06
100	7.70332337591188e-06	0.00151209677419355	7.72662334237396e-06
101	7.77061032877868e-06	0.00149700598802395	7.79390239273568e-06
102	7.26611651711332e-06	0.00148221343873518	7.28770828216044e-06
103	7.45835128252988e-06	0.00146771037181996	7.48022200618493e-06
104	8.35016755943253e-06	0.00145348837209302	8.37440743085957e-06
105	7.43126522386843e-06	0.00143953934740883	7.45273152667692e-06
106	7.44408841897061e-06	0.00142585551330798	7.46532619386115e-06
107	7.32708424953807e-06	0.00141242937853107	7.34778135680631e-06
108	8.03516102147666e-06	0.00139925373134328	8.05759466548084e-06
109	7.59136689372437e-06	0.00138632162661738	7.61240837456139e-06
110	7.51834097527367e-06	0.00137362637362637	7.53894550590430e-06
111	6.79312082821262e-06	0.00136116152450091	6.81162053185214e-06
112	7.41903647469240e-06	0.00134892086330935	7.43907578044931e-06
113	7.43713921648268e-06	0.00133689839572193	7.45702875255079e-06
114	7.74297625159641e-06	0.00132508833922261	7.76351768018418e-06
115	7.40773293245163e-06	0.00131348511383538	7.42718964629974e-06
116	7.44715861207857e-06	0.00130208333333333	7.46654393552647e-06
117	7.34601310787024e-06	0.00129087779690189	7.36497963630421e-06
118	7.04334368873795e-06	0.00127986348122867	7.06134618781505e-06
119	7.21651474275036e-06	0.00126903553299492	7.23484735730376e-06
120	6.80447104513461e-06	0.00125838926174497	6.82157309068714e-06
121	7.55559231593615e-06	0.00124792013311148	7.57446557591166e-06
122	7.71680485406954e-06	0.00123762376237624	7.73593745096131e-06
123	7.78664696269913e-06	0.00122749590834697	7.80575429999978e-06
124	8.29393923180817e-06	0.00121753246753247	8.31417745918219e-06
125	7.51452158069297e-06	0.00120772946859903	7.53272501262534e-06
126	7.70014705979915e-06	0.00119808306709265	7.71863881221756e-06
127	7.83806555737948e-06	0.00118858954041204	7.85664156949271e-06
128	6.84124942309299e-06	0.00117924528301887	6.85738720246422e-06
129	7.86627508559796e-06	0.00117004680187208	7.88464658261441e-06
130	7.95945382036031e-06	0.00116099071207430	7.97791281888485e-06
131	7.53056472007212e-06	0.00115207373271889	7.54791255324643e-06
132	7.70151385536425e-06	0.00114329268292683	7.71912835141871e-06
133	7.20057129562473e-06	0.00113464447806354	7.21691163180284e-06
134	7.42286969418872e-06	0.00112612612612613	7.43960359289913e-06
135	7.05563398170765e-06	0.00111773472429210	7.07137584615641e-06
136	6.97491445312147e-06	0.00110946745562130	6.99038416261188e-06
137	7.59996563332142e-06	0.00110132158590308	7.61674016578908e-06
138	7.50919219353500e-06	0.00109329446064140	7.52562096444220e-06
139	8.18748817731043e-06	0.00108538350217077	8.20527356811560e-06
140	8.28163689627590e-06	0.00107758620689655	8.29946038633091e-06
141	7.47653099595865e-06	0.00106990014265335	7.49250670131248e-06
142	7.22904053057288e-06	0.00106232294617564	7.24444694403706e-06
143	7.45560535956019e-06	0.00105485232067511	7.47134887201839e-06
144	7.60003290160983e-06	0.00104748603351955	7.61595220482646e-06
145	7.35828716523508e-06	0.00104022191400832	7.37357965340860e-06
146	7.81491191821371e-06	0.00103305785123967	7.83105032085912e-06
147	7.62507090837087e-06	0.00102599179206566	7.64072621086584e-06
148	7.59544963760022e-06	0.00101902173913043	7.61093533259556e-06
149	8.05075162152398e-06	0.00101214574898785	8.06702989668303e-06
150	6.85322408287128e-06	0.00100536193029491	6.86699286155308e-06
151	7.20271496452528e-06	0.000998668442077230	7.21712225210307e-06
152	7.66459505657886e-06	0.000992063492063492	7.67979737148313e-06
153	6.80191221433715e-06	0.000985545335085414	6.81528978297047e-06
154	7.11216150152960e-06	0.000979112271540470	7.12605138127785e-06
155	7.34663428459554e-06	0.000972762645914397	7.36092133989051e-06
156	7.52795313146491e-06	0.000966494845360825	7.54249767041023e-06
157	7.68035638576453e-06	0.000960307298335467	7.69509662922265e-06
158	7.58895257956952e-06	0.000954198473282443	7.60341531933585e-06
159	8.31220854757336e-06	0.000948166877370417	8.32795158200449e-06
160	8.03463297146619e-06	0.000942211055276382	8.04976339450340e-06
161	7.93664248574576e-06	0.000936329588014981	7.95150204030527e-06
162	8.21501534554636e-06	0.000930521091811414	8.23030903354580e-06
163	7.89452971559114e-06	0.000924784217016030	7.90913073015768e-06
164	6.87843872512945e-06	0.000919117647058823	6.89110749025914e-06
165	7.60479173034952e-06	0.000913520097442144	7.61871139221262e-06
166	7.49033745767184e-06	0.000907990314769976	7.50392054565188e-06
167	7.18582118295035e-06	0.000902527075812274	7.19876514948245e-06
168	7.61032652655224e-06	0.000897129186602871	7.62399024473778e-06
169	7.13833118111802e-06	0.000891795481569560	7.15108134943944e-06
170	8.33507671269591e-06	0.000886524822695035	8.34986483653498e-06
171	8.22947098313310e-06	0.000881316098707403	8.24401077713060e-06
172	8.35128175658183e-06	0.000876168224299065	8.36599145403087e-06
173	6.36292944032678e-06	0.000871080139372822	6.37402442379425e-06
174	8.63663090930299e-06	0.000866050808314088	8.65155760173408e-06
175	7.82434978926202e-06	0.000861079219288175	7.83784466370838e-06
176	7.66138573903545e-06	0.000856164383561644	7.67450790718243e-06
177	7.99752349090143e-06	0.000851305334846765	8.01109940966754e-06
178	7.62695663288345e-06	0.000846501128668172	7.63992222750955e-06
179	7.28588397111336e-06	0.000841750841750842	7.29815055224201e-06
180	7.71458534539757e-06	0.000837053571428572	7.72751925914010e-06
181	7.27367158109514e-06	0.000832408435072142	7.28581149157317e-06
182	7.86853272053481e-06	0.000827814569536424	7.88166840820533e-06
183	6.99604649252698e-06	0.000823271130625686	7.00752343061935e-06
184	8.12531573313586e-06	0.000818777292576419	8.13862128469145e-06
185	7.53661864026233e-06	0.000814332247557003	7.54887779734610e-06
186	7.00141805345345e-06	0.000809935205183585	7.01271306470049e-06
187	7.63657218380707e-06	0.000805585392051558	7.64886989528144e-06
188	7.69722897950971e-06	0.000801282051282051	7.70956430389886e-06
189	7.92886957812901e-06	0.000797024442082891	7.94145285209934e-06
190	8.24367385353642e-06	0.000792811839323467	8.25672677009442e-06
191	8.28841195411260e-06	0.000788643533123028	8.30148459234535e-06
192	7.28089587115397e-06	0.000784518828451883	7.29233538257539e-06
193	7.60287022030289e-06	0.000780437044745057	7.61474201553846e-06
194	7.63985321158384e-06	0.000776397515527950	7.65168384799501e-06
195	7.64395832590566e-06	0.000772399588053553	7.65571356947615e-06
196	7.94003597363205e-06	0.000768442622950820	7.95220406929101e-06
197	7.69872714507320e-06	0.000764525993883792	7.71051579396056e-06
198	7.96766375832979e-06	0.000760649087221095	7.97977347596655e-06
199	7.16906234981360e-06	0.000756811301715439	7.17992670864024e-06
200	8.27131893014094e-06	0.000753012048192771	8.28378191922980e-06

==> experiments/linearsqrroot.tex <==
n err bound boundsharp
1	8.75128831437271e-05	0.00242592697397690	8.79384319177228e-05
2	8.30669053100085e-05	0.00316618769702135	8.35940265166061e-05
3	7.58565443474324e-05	0.00376011670070774	7.64273153901104e-05
4	8.50007626563619e-05	0.00427226317192790	8.57299960919611e-05
5	8.54572193975716e-05	0.00472988199043560	8.62642291576097e-05
6	8.43102506852644e-05	0.00514769858416551	8.51749949192643e-05
7	8.41347067739944e-05	0.00553477512912865	8.50695809422486e-05
8	8.21111452166437e-05	0.00589716957091894	8.30848446925418e-05
9	7.92894197048296e-05	0.00623917268912867	8.02764734341429e-05
10	8.89419695404598e-05	0.00656395692372024	9.01098994936888e-05
11	8.52293283689409e-05	0.00687394711491733	8.64038560165218e-05
12	8.88256278242063e-05	0.00717104650997755	9.00979105791664e-05
13	8.54023461983576e-05	0.00745678172479966	8.66786605137950e-05
14	8.29235763001443e-05	0.00773239962325114	8.41983270512151e-05
15	8.95720345082864e-05	0.00799893429925836	9.10049088017477e-05
16	8.35875415359977e-05	0.00825725473032173	8.49679400350662e-05
17	8.59602348635013e-05	0.00850809951706352	8.74213021789647e-05
18	8.73569020491300e-05	0.00875210274793586	8.88866250115365e-05
19	9.39754046021334e-05	0.00898981361405444	9.56622257100833e-05
20	9.50158755794481e-05	0.00922171152755766	9.67668375017746e-05
21	8.72373230626312e-05	0.00944821794328112	8.88862126362408e-05
22	9.05102465647358e-05	0.00966970572241212	9.22672464124257e-05
23	9.07721652289901e-05	0.00988650663561980	9.25692779112487e-05
24	8.61462004775293e-05	0.0100989174386700	8.78849226872699e-05
25	8.03704259030521e-05	0.0103072048391961	8.20285424823277e-05
26	8.04744083418992e-05	0.0105116095924627	8.21666394296726e-05
27	8.86484739511927e-05	0.0107123499059011	9.05537265694033e-05
28	7.94327982004489e-05	0.0109096242899069	8.11668941851550e-05
29	7.64904775276771e-05	0.0111036139611851	7.81920582249921e-05
30	9.00802662565048e-05	0.0112944848816239	9.21207142084630e-05
31	8.23554753624011e-05	0.0114823894980702	8.42438673781141e-05
32	8.77356112436372e-05	0.0116674682349666	8.97886626583063e-05
33	8.35371641093888e-05	0.0118498507814511	8.55139776605683e-05
34	9.48557984728565e-05	0.0120296572065042	9.71345008417202e-05
35	9.16422655011087e-05	0.0122069989294097	9.38804962469733e-05
36	8.45484396983556e-05	0.0123819795678448	8.66475151262461e-05
37	8.24845691225548e-05	0.0125546956819436	8.45545580112056e-05
38	8.07164297570939e-05	0.0127252374295237	8.27750038873860e-05
39	8.16659013413647e-05	0.0128936891451043	8.37697892741370e-05
40	8.38242906360159e-05	0.0130601298532805	8.60213564116557e-05
41	8.51136708174293e-05	0.0132246337253268	8.73680409113155e-05
42	8.37172924235035e-05	0.0133872704865223	8.59513919406514e-05
43	8.68167275654033e-05	0.0135481057805425	8.91722269306479e-05
44	9.13416084474607e-05	0.0137072014963291	9.38433600809319e-05
45	8.56675903175129e-05	0.0138646160620491	8.80351265108347e-05
46	8.26583787656837e-05	0.0140204047101089	8.49757651804521e-05
47	8.33600275626939e-05	0.0141746197166325	8.57268610315878e-05
48	9.61378612481791e-05	0.0143273106183467	9.88938040062580e-05
49	8.65082902827752e-05	0.0144785244094270	8.90114654996777e-05
50	8.93043312433440e-05	0.0146283057205212	9.19157335784446e-05
51	8.59966895378139e-05	0.0147766969818845	8.85379888749714e-05
52	8.10924036838066e-05	0.0149237385723156	8.35047968998057e-05
53	8.64845483709925e-05	0.0150694689553788	8.90853473090674e-05
54	8.74567667405355e-05	0.0152139248042091	9.01154985388999e-05
55	8.80245265474812e-05	0.0153571411160520	9.07301854706619e-05
56	8.45052538924430e-05	0.0154991513175522	8.71271059002551e-05
57	8.44459761691441e-05	0.0156399873616859	8.70871638705937e-05
58	8.55690212505480e-05	0.0157796798171338	8.82679898950752e-05
59	7.91601370349161e-05	0.0159182579508043	8.16779559728324e-05
60	8.89952193624084e-05	0.0160557498041393	9.18496756651468e-05
61	8.61285870929300e-05	0.0161921822637583	8.89193572662889e-05
62	9.72412818127700e-05	0.0163275811269590	0.000100407287772560
63	7.92635718549583e-05	0.0164619711625095	8.18761887125731e-05
64	9.08533589510116e-05	0.0165953761671522	9.38743310884384e-05
65	7.90777982194986e-05	0.0167278190181760	8.17261805847752e-05
66	8.58057020415517e-05	0.0168593217223906	8.87028455766781e-05
67	9.32901363988784e-05	0.0169899054617918	9.64636415880880e-05
68	9.21957271770245e-05	0.0171195906361990	9.53560715787542e-05
69	8.79162117145297e-05	0.0172483969030958	9.09510444027744e-05
70	8.22433567745692e-05	0.0173763432148996	8.51028697589875e-05
71	7.79447045818872e-05	0.0175034478538612	8.06718369087980e-05
72	8.48952990306372e-05	0.0176297284647700	8.78893011245483e-05
73	8.26139977260561e-05	0.0177552020856427	8.55523565552539e-05
74	7.96256161528687e-05	0.0178798851765310	8.24751888203472e-05
75	8.80560053984294e-05	0.0180037936465982	9.12234919100646e-05
76	8.86953255095089e-05	0.0181269428795846	9.19074357246250e-05
77	9.09985936437025e-05	0.0182493477577816	9.43154929209417e-05
78	9.15710714735415e-05	0.0183710226846162	9.49359960613226e-05
79	9.13248410257771e-05	0.0184919816059411	9.46996965020558e-05
80	8.44946496570089e-05	0.0186122380301319	8.76320100663693e-05
81	8.79378338420798e-05	0.0187318050470512	9.12301620389011e-05
82	8.82373199584679e-05	0.0188506953459815	9.15632026121125e-05
83	8.45523000580402e-05	0.0189689212325706	8.77626824647774e-05
84	9.00969007005424e-05	0.0190864946448752	9.35344242603747e-05
85	8.77256928666365e-05	0.0192034271685484	9.10970090221871e-05
86	8.65423978564110e-05	0.0193197300512288	8.98879909261393e-05
87	8.45500791936509e-05	0.0194354142161852	8.78323390063423e-05
88	8.60083618409968e-05	0.0195504902752598	8.93695737372435e-05
89	9.16344525247269e-05	0.0196649685411546	9.52368465476877e-05
90	8.43277360558928e-05	0.0197788590391068	8.76632191029093e-05
91	8.63652310032601e-05	0.0198921715179733	8.97984538430734e-05
92	9.33878670859429e-05	0.0200049154607842	9.71273885360049e-05
93	8.51169004605817e-05	0.0201171000947776	8.85404073303977e-05
94	8.38230221841346e-05	0.0202287344009520	8.72113203399690e-05
95	7.83041541902388e-05	0.0203398271231640	8.14894217496051e-05
96	8.79692506937484e-05	0.0204503867768077	9.15699578373845e-05
97	8.60916053201340e-05	0.0205604216570761	8.96362375178080e-05
98	8.60618465309018e-05	0.0206699398468533	8.96170359530739e-05
99	8.67830623910345e-05	0.0207789492242388	9.04050871814018e-05
100	8.43296479637688e-05	0.0208874574697405	8.78438239822366e-05
101	8.91605473571845e-05	0.0209954720731384	9.29129913307025e-05
102	9.11967368375172e-05	0.0211030003400499	9.50423026236287e-05
103	8.56527099853475e-05	0.0212100493982061	8.92879902647646e-05
104	8.63090286800345e-05	0.0213166262034528	8.99957061980231e-05
105	8.66986256342492e-05	0.0214227375454996	9.04169630470505e-05
106	8.38428465225496e-05	0.0215283900534193	8.74457630340666e-05
107	8.28370044766286e-05	0.0216335902009160	8.64264245686737e-05
108	8.39662714004000e-05	0.0217383443113744	8.76096811503895e-05
109	8.52277979379879e-05	0.0218426585627030	8.89486723729233e-05
110	9.40408846212920e-05	0.0219465389919700	9.81638751853002e-05
111	8.62258027764709e-05	0.0220499914998601	9.00238923114379e-05
112	9.00361940510365e-05	0.0221530218549488	9.40235958996132e-05
113	9.69053575354907e-05	0.0222556356977999	0.000101210282450279
114	8.80800204469936e-05	0.0223578385449105	9.20229887415844e-05
115	9.42909121941901e-05	0.0224596357924959	9.85265009131247e-05
116	9.20632964240649e-05	0.0225610327201275	9.62100914107423e-05
117	8.50919704568029e-05	0.0226620344942342	8.89488656606146e-05
118	8.19323002382887e-05	0.0227626461714585	8.56683852238757e-05
119	8.31751676416073e-05	0.0228628727019040	8.69815533051935e-05
120	8.31569732713746e-05	0.0229627189322465	8.69779986180228e-05
121	8.46083433344973e-05	0.0230621896087296	8.85053142301515e-05
122	8.67378110819015e-05	0.0231612893800593	9.07565560609216e-05
123	8.85983502697118e-05	0.0232600228001827	9.27231680443348e-05
124	8.37880305770159e-05	0.0233583943309667	8.77043751671790e-05
125	9.01827980223842e-05	0.0234564083447933	9.44175172174160e-05
126	8.18749589218643e-05	0.0235540691270367	8.57389567803362e-05
127	8.35831053815497e-05	0.0236513808784751	8.75381600462362e-05
128	9.03743705446332e-05	0.0237483477176151	9.46710804190883e-05
129	8.65849159848279e-05	0.0238449736829132	9.07171241236104e-05
130	8.77053543938360e-05	0.0239412627349506	9.19009562939548e-05
131	9.30815051211832e-05	0.0240372187585156	9.75487085847179e-05
132	8.31320022748273e-05	0.0241328455646097	8.71414624707610e-05
133	8.06037623287451e-05	0.0242281468924072	8.45048370969599e-05
134	9.20207758526759e-05	0.0243231264111228	9.65015869826598e-05
135	8.85188077361406e-05	0.0244177877218380	9.28486399219218e-05
136	9.39797750356602e-05	0.0245121343592582	9.85914993475268e-05
137	8.72223105846347e-05	0.0246061697934063	9.15089283513174e-05
138	9.11012024471739e-05	0.0246998974312709	9.56075288510157e-05
139	9.35472437037557e-05	0.0247933206183992	9.81848475863622e-05
140	9.16532967261585e-05	0.0248864426404348	9.62125366720155e-05
141	8.64762785457750e-05	0.0249792667246030	9.08025538340448e-05
142	9.48971385818773e-05	0.0250717960411621	9.96641367059773e-05
143	8.91540864903010e-05	0.0251640337047970	9.36361707708037e-05
144	7.67337703395502e-05	0.0252559827759698	8.06159016866590e-05
145	7.77840368527444e-05	0.0253476462622380	8.17198748730992e-05
146	9.36228253579154e-05	0.0254390271195202	9.83833624114016e-05
147	9.54008998487159e-05	0.0255301282533304	0.000100276332839557
148	9.11945978411258e-05	0.0256209525199727	9.58622015026578e-05
149	8.09600167538636e-05	0.0257115027276991	8.51168969621830e-05
150	8.74463205508773e-05	0.0258017816378349	9.19470784038838e-05
151	9.19354304849881e-05	0.0258917919658660	9.66979976104178e-05
152	9.17168895324494e-05	0.0259815363824956	9.64854869827011e-05
153	8.45542398073627e-05	0.0260710175146773	8.89575504242246e-05
154	8.89325209352405e-05	0.0261602379466069	9.35824200110315e-05
155	8.18285111652723e-05	0.0262492002206866	8.61297493953469e-05
156	9.33628391273986e-05	0.0263379068384721	9.82809762765651e-05
157	9.64031679469547e-05	0.0264263602615789	0.000101516902401851
158	7.91772305164562e-05	0.0265145629125749	8.33768398231167e-05
159	9.51186148682295e-05	0.0266025171758329	0.000100189122468168
160	9.17246293529377e-05	0.0266902253983797	9.66100138231593e-05
161	9.10418066169985e-05	0.0267776898906958	9.59216240740879e-05
162	8.81050960303145e-05	0.0268649129275201	9.28499984143576e-05
163	8.48331232751589e-05	0.0269518967486086	8.94096522615121e-05
164	9.89266970590567e-05	0.0270386435594892	0.000104255946599147
165	9.41300687188679e-05	0.0271251555321857	9.92278861198233e-05
166	9.39172947063760e-05	0.0272114348059263	9.90147769113707e-05
167	8.36949136140202e-05	0.0272974834878315	8.82793943335700e-05
168	8.77953102610969e-05	0.0273833036535879	9.26027819552750e-05
169	8.60620353616061e-05	0.0274688973480950	9.07955738584849e-05
170	8.78260143113961e-05	0.0275542665861080	9.26847863336248e-05
171	7.95699202085699e-05	0.0276394133528458	8.39742358113678e-05
172	8.72303995502670e-05	0.0277243396046003	9.20574191970603e-05
173	8.79243708976120e-05	0.0278090472693247	9.28008553988467e-05
174	8.62237972633581e-05	0.0278935382471985	9.10377802853014e-05
175	8.25727291299758e-05	0.0279778144111844	8.71994386487058e-05
176	9.06562870357712e-05	0.0280618776075777	9.57402721556736e-05
177	9.47931759150525e-05	0.0281457296565254	0.000100122620526500
178	7.39246671986403e-05	0.0282293723525512	7.81026999649096e-05
179	8.28728553478446e-05	0.0283128074650450	8.75756961782834e-05
180	8.48445482182689e-05	0.0283960367387674	8.96698989236691e-05
181	9.00823750697783e-05	0.0284790618943104	9.52134965867889e-05
182	9.37575650496367e-05	0.0285618846285814	9.91122331066235e-05
183	8.53237607701034e-05	0.0286445066152398	9.02192718720189e-05
184	8.22186313256431e-05	0.0287269295051508	8.69490050799264e-05
185	8.10234137859551e-05	0.0288091549268168	8.56937791657489e-05
186	8.26615927955924e-05	0.0288911844867880	8.74467209811218e-05
187	9.39520280058676e-05	0.0289730197700961	9.93743302409019e-05
188	8.96268652563088e-05	0.0290546623406273	9.48481603893761e-05
189	8.65955483654613e-05	0.0291361137415428	9.16314625559264e-05
190	7.63877948725729e-05	0.0292173754956370	8.08522309190549e-05
191	8.69927402906915e-05	0.0292984491057318	9.20834024393413e-05
192	8.12679623243161e-05	0.0293793360550229	8.60137930563507e-05
193	9.64829560234988e-05	0.0294600378074533	0.000102178451209498
194	9.04385695124121e-05	0.0295405558080500	9.57721428694963e-05
195	8.15195156941951e-05	0.0296208914832655	8.63572796038037e-05
196	8.87879227634434e-05	0.0297010462413175	9.40670085776387e-05
197	9.23462198677606e-05	0.0297810214725015	9.78331697815741e-05
198	9.16734032470136e-05	0.0298608185495205	9.71513570555702e-05
199	8.44272796643574e-05	0.0299404388277879	8.94881071756128e-05
200	9.39613183808356e-05	0.0299404388277879	9.95912035859063e-05

==> experiments/quadraticequi.tex <==
n err bound boundsharp
1	2.67992852459501e-10	1.00300835606217e-06	5.80968745540816e-09
2	4.51594500366095e-10	1.00300835606217e-06	5.51033127859144e-09
3	2.76942181286220e-10	1.00300835606217e-06	5.23157757332831e-09
4	3.37345627705546e-10	1.00300835606217e-06	5.99432169372302e-09
5	5.92764492019991e-10	1.00300835606217e-06	5.18725752193348e-09
6	2.20628483963532e-10	1.00300835606217e-06	5.38133562377305e-09
7	3.74363780947976e-10	1.00300835606217e-06	5.16107326634274e-09
8	1.93576128654065e-10	1.00300835606217e-06	5.60413911299100e-09
9	4.28937062866029e-10	1.00300835606217e-06	5.30804375303530e-09
10	5.80035489655614e-10	1.00300835606217e-06	5.73747957477317e-09
11	5.98190140886107e-10	1.00300835606217e-06	5.73566914130162e-09
12	5.94165699199106e-10	1.00300835606217e-06	5.25336740554818e-09
13	3.59096638287403e-10	1.00300835606217e-06	5.27877861618910e-09
14	4.27655904410320e-10	1.00300835606217e-06	5.79458138344942e-09
15	4.06631033456586e-10	1.00300835606217e-06	5.65193033197279e-09
16	2.92906201877550e-10	1.00300835606217e-06	5.46378148983944e-09
17	3.44870067142885e-10	1.00300835606217e-06	5.29983997066294e-09
18	2.38202072516744e-10	1.00300835606217e-06	5.45847996782213e-09
19	5.52909229725271e-10	1.00300835606217e-06	5.77683511415663e-09
20	6.90254208970919e-10	1.00300835606217e-06	5.08418511580026e-09
21	2.69606805629177e-10	1.00300835606217e-06	5.48027416198995e-09
22	2.95234125460337e-10	1.00300835606217e-06	5.65446683338967e-09
23	2.68961682605986e-10	1.00300835606217e-06	5.60104224250591e-09
24	2.94988862415893e-10	1.00300835606217e-06	5.59494022702516e-09
25	3.80223420765860e-10	1.00300835606217e-06	5.84136969293208e-09
26	2.86073854801644e-10	1.00300835606217e-06	5.50370085311664e-09
27	4.10415161025759e-10	1.00300835606217e-06	5.23410523776760e-09
28	3.15764252561880e-10	1.00300835606217e-06	5.24186535153917e-09
29	3.11633165236728e-10	1.00300835606217e-06	5.24804045035002e-09
30	4.73717377159850e-10	1.00300835606217e-06	5.54620155636249e-09
31	1.78809099530494e-10	1.00300835606217e-06	5.51256534545801e-09
32	2.70038097046197e-10	1.00300835606217e-06	5.57284380201767e-09
33	6.04460959859908e-10	1.00300835606217e-06	5.64754068157937e-09
34	5.27365978009458e-10	1.00300835606217e-06	4.99239590655408e-09
35	4.56953720427136e-10	1.00300835606217e-06	5.52896124982886e-09
36	2.14162047090204e-10	1.00300835606217e-06	5.25363599222854e-09
37	2.25202475897760e-10	1.00300835606217e-06	5.92807451667213e-09
38	4.65822197324557e-10	1.00300835606217e-06	5.71269701607969e-09
39	3.27331247104493e-10	1.00300835606217e-06	5.56947759999115e-09
40	4.42682992998412e-10	1.00300835606217e-06	5.52212409798234e-09
41	2.62147642461652e-10	1.00300835606217e-06	5.57586085689116e-09
42	2.69093140227861e-10	1.00300835606217e-06	5.16593749832985e-09
43	3.67569841036166e-10	1.00300835606217e-06	6.06283729207658e-09
44	2.89777370130486e-10	1.00300835606217e-06	5.05832088769273e-09
45	3.65911712261550e-10	1.00300835606217e-06	5.51435300152758e-09
46	2.58936087734580e-10	1.00300835606217e-06	5.58680797047784e-09
47	4.02639807858617e-10	1.00300835606217e-06	5.65143803462579e-09
48	3.03959595388035e-10	1.00300835606217e-06	5.40604248433930e-09
49	1.87839968811948e-10	1.00300835606217e-06	4.77622584413709e-09
50	3.65939651291490e-10	1.00300835606217e-06	5.69504919280487e-09
51	1.45146386451103e-10	1.00300835606217e-06	5.45407826562320e-09
52	3.14671574401916e-10	1.00300835606217e-06	5.38293202939067e-09
53	3.12242477446237e-10	1.00300835606217e-06	5.65400062823347e-09
54	2.87448380629827e-10	1.00300835606217e-06	5.59635493986767e-09
55	2.66039262442717e-10	1.00300835606217e-06	5.87650193689677e-09
56	3.65691002260460e-10	1.00300835606217e-06	5.25052082858200e-09
57	3.28611328988462e-10	1.00300835606217e-06	5.35706095315990e-09
58	2.44144314895867e-10	1.00300835606217e-06	6.04042349160784e-09
59	3.48184729115381e-10	1.00300835606217e-06	5.69526690595556e-09
60	3.05679219336867e-10	1.00300835606217e-06	5.72609808333028e-09
61	2.47289998514243e-10	1.00300835606217e-06	5.02451424506874e-09
62	2.12598987699440e-10	1.00300835606217e-06	5.11612556130001e-09
63	3.39473174111854e-10	1.00300835606217e-06	5.14793259986598e-09
64	1.70928841775187e-10	1.00300835606217e-06	5.29406145509821e-09
65	2.44336771229824e-10	1.00300835606217e-06	5.32423339042156e-09
66	2.80949898795372e-10	1.00300835606217e-06	5.59033519696883e-09
67	2.33072355704902e-10	1.00300835606217e-06	5.58367065521125e-09
68	2.55823408619089e-10	1.00300835606217e-06	5.74524319650316e-09
69	3.78707474490534e-10	1.00300835606217e-06	5.36573591417405e-09
70	2.25426975824613e-10	1.00300835606217e-06	4.93660594304817e-09
71	2.45189934148333e-10	1.00300835606217e-06	5.78995230801776e-09
72	3.11875588597949e-10	1.00300835606217e-06	5.98271745171299e-09
73	1.38560562779698e-10	1.00300835606217e-06	5.26892141227850e-09
74	3.64917216292562e-10	1.00300835606217e-06	5.64557677961559e-09
75	2.84738440092200e-10	1.00300835606217e-06	5.71941697842338e-09
76	2.69236468852488e-10	1.00300835606217e-06	5.69336668603062e-09
77	2.12052607098151e-10	1.00300835606217e-06	4.83230506767293e-09
78	3.65080343166249e-10	1.00300835606217e-06	6.12390920226821e-09
79	5.46326008130769e-10	1.00300835606217e-06	5.52533436600574e-09
80	3.53670882429428e-10	1.00300835606217e-06	5.80117323897868e-09
81	1.94422055703106e-10	1.00300835606217e-06	5.26645944584310e-09
82	3.12115578356849e-10	1.00300835606217e-06	5.38807961463210e-09
83	2.17503525485692e-10	1.00300835606217e-06	5.31180335205221e-09
84	1.74322217240467e-10	1.00300835606217e-06	5.40713784420689e-09
85	1.90772622348135e-10	1.00300835606217e-06	5.77047811290164e-09
86	2.14123208618229e-10	1.00300835606217e-06	5.30595850661893e-09
87	2.39457865198402e-10	1.00300835606217e-06	5.25700429866468e-09
88	1.74307525627808e-10	1.00300835606217e-06	5.20730395836688e-09
89	8.88668943666688e-11	1.00300835606217e-06	5.46309077167430e-09
90	2.09193394465529e-10	1.00300835606217e-06	5.34034633737745e-09
91	2.11629155119696e-10	1.00300835606217e-06	5.35734448738110e-09
92	2.96744706850709e-10	1.00300835606217e-06	5.62458708522691e-09
93	1.74605223998690e-10	1.00300835606217e-06	5.99294946390402e-09
94	1.86548048223482e-10	1.00300835606217e-06	5.41536306175724e-09
95	2.55203481371786e-10	1.00300835606217e-06	5.72194241830533e-09
96	2.30377710597546e-10	1.00300835606217e-06	5.37676202447315e-09
97	2.07396376187807e-10	1.00300835606217e-06	5.73675210797537e-09
98	2.45958422755810e-10	1.00300835606217e-06	5.51965138329113e-09
99	2.69102367457125e-10	1.00300835606217e-06	5.59583344818939e-09
100	1.53054843284124e-10	1.00300835606217e-06	5.66340310903921e-09
101	2.37054906699688e-10	1.00300835606217e-06	5.67970435006764e-09
102	1.82326246076781e-10	1.00300835606217e-06	5.47071690711979e-09
103	1.94229007397636e-10	1.00300835606217e-06	5.18444001729274e-09
104	3.36170374122639e-10	1.00300835606217e-06	5.51976340835183e-09
105	2.19176961858168e-10	1.00300835606217e-06	5.12026642003151e-09
106	3.22615290380811e-10	1.00300835606217e-06	5.65426241140934e-09
107	2.10507254185073e-10	1.00300835606217e-06	5.47840315469102e-09
108	2.07233455313445e-10	1.00300835606217e-06	5.67745251816028e-09
109	1.75965982466544e-10	1.00300835606217e-06	5.18264312784377e-09
110	1.21783888428586e-10	1.00300835606217e-06	5.11408421098600e-09
111	1.56025248763727e-10	1.00300835606217e-06	5.78906622774343e-09
112	3.66775839923697e-10	1.00300835606217e-06	5.95391175606806e-09
113	2.40472668150542e-10	1.00300835606217e-06	5.13970791677421e-09
114	2.05505549120512e-10	1.00300835606217e-06	5.57082850496160e-09
115	1.86637011988573e-10	1.00300835606217e-06	6.04101130432822e-09
116	1.42714360174581e-10	1.00300835606217e-06	6.09406678485966e-09
117	1.67539758527820e-10	1.00300835606217e-06	6.12607322266344e-09
118	2.26631977480376e-10	1.00300835606217e-06	5.64901248615938e-09
119	1.81462393262043e-10	1.00300835606217e-06	5.05707659917629e-09
120	1.93607982043773e-10	1.00300835606217e-06	5.72948672515142e-09
121	2.37986523837466e-10	1.00300835606217e-06	5.91234687250567e-09
122	2.34716874258589e-10	1.00300835606217e-06	5.62757908950459e-09
123	3.93211336603113e-10	1.00300835606217e-06	6.16970202066858e-09
124	2.05033927356033e-10	1.00300835606217e-06	5.54400522112916e-09
125	2.78141966508011e-10	1.00300835606217e-06	5.43904632203105e-09
126	3.74967747803842e-10	1.00300835606217e-06	5.74775169154336e-09
127	1.48826812958330e-10	1.00300835606217e-06	5.62108802680064e-09
128	2.93721578378042e-10	1.00300835606217e-06	5.57306644307977e-09
129	3.02645608441228e-10	1.00300835606217e-06	5.56785571926080e-09
130	1.75553772413798e-10	1.00300835606217e-06	5.73704885997198e-09
131	1.70767731022169e-10	1.00300835606217e-06	5.71330519967943e-09
132	1.94287824061617e-10	1.00300835606217e-06	5.47925171249379e-09
133	1.43242839976686e-10	1.00300835606217e-06	5.66415064730843e-09
134	1.76288001690886e-10	1.00300835606217e-06	5.11367981986594e-09
135	3.08829000574953e-10	1.00300835606217e-06	5.67869622888060e-09
136	2.94208124604176e-10	1.00300835606217e-06	5.31510451381848e-09
137	2.75470950657613e-10	1.00300835606217e-06	5.51139769875765e-09
138	2.71444511702626e-10	1.00300835606217e-06	5.53233446295053e-09
139	3.28680863176621e-10	1.00300835606217e-06	5.54739375401318e-09
140	3.58934957355210e-10	1.00300835606217e-06	5.93944117562336e-09
141	3.04323534731639e-10	1.00300835606217e-06	5.48474085769027e-09
142	2.92191419899756e-10	1.00300835606217e-06	5.75848576822275e-09
143	2.32456164770634e-10	1.00300835606217e-06	5.46182741154955e-09
144	1.50371592991645e-10	1.00300835606217e-06	5.25462452179756e-09
145	2.94092408605092e-10	1.00300835606217e-06	5.62972136478847e-09
146	2.52228946609073e-10	1.00300835606217e-06	5.40864333250798e-09
147	1.95859891350163e-10	1.00300835606217e-06	5.66922885348188e-09
148	4.41798221230443e-10	1.00300835606217e-06	5.84512825285865e-09
149	3.16655078998737e-10	1.00300835606217e-06	5.93376359524188e-09
150	3.08617809874501e-10	1.00300835606217e-06	5.42777317269445e-09
151	2.98098508121111e-10	1.00300835606217e-06	5.97992921290253e-09
152	1.50103626050287e-10	1.00300835606217e-06	5.59534983171658e-09
153	1.73683672432589e-10	1.00300835606217e-06	5.21115890117365e-09
154	3.70683171842798e-10	1.00300835606217e-06	5.80364108504901e-09
155	3.13370183308687e-10	1.00300835606217e-06	5.54639154682355e-09
156	2.57604283965520e-10	1.00300835606217e-06	5.35253781292959e-09
157	3.66498314881918e-10	1.00300835606217e-06	5.62129281247133e-09
158	1.94405463763895e-10	1.00300835606217e-06	5.84562691897105e-09
159	2.67801652267583e-10	1.00300835606217e-06	5.81986405766028e-09
160	3.55385773267548e-10	1.00300835606217e-06	5.36093587704282e-09
161	1.98216000276590e-10	1.00300835606217e-06	5.66550019619746e-09
162	2.43532334706374e-10	1.00300835606217e-06	5.23686109584782e-09
163	3.76520162870415e-10	1.00300835606217e-06	5.77117406372573e-09
164	2.51692204564196e-10	1.00300835606217e-06	6.09269090987951e-09
165	4.49462964183098e-10	1.00300835606217e-06	5.36369020640074e-09
166	1.96144585645642e-10	1.00300835606217e-06	5.35136744483136e-09
167	3.50423677084004e-10	1.00300835606217e-06	5.56859218382988e-09
168	2.64232614542773e-10	1.00300835606217e-06	5.57176591178201e-09
169	2.58790506383639e-10	1.00300835606217e-06	5.61536906015434e-09
170	1.43872572374293e-10	1.00300835606217e-06	4.88058162436842e-09
171	3.74260018305843e-10	1.00300835606217e-06	5.35432363711516e-09
172	4.09841192014778e-10	1.00300835606217e-06	5.60137140424321e-09
173	4.05559164901743e-10	1.00300835606217e-06	5.65945673390087e-09
174	3.76700478409251e-10	1.00300835606217e-06	6.06560916055512e-09
175	2.98071353387180e-10	1.00300835606217e-06	5.35519738746670e-09
176	2.41471282972523e-10	1.00300835606217e-06	5.34338961901938e-09
177	4.74888457572824e-10	1.00300835606217e-06	5.32188249637755e-09
178	4.99124756982997e-10	1.00300835606217e-06	5.68808545385490e-09
179	2.93601391263779e-10	1.00300835606217e-06	5.58939379403244e-09
180	3.91961632175941e-10	1.00300835606217e-06	5.94349125000425e-09
181	4.10268075333813e-10	1.00300835606217e-06	5.40814711682727e-09
182	3.44658554118082e-10	1.00300835606217e-06	5.38433355771351e-09
183	5.21697437252368e-10	1.00300835606217e-06	5.51991216667597e-09
184	4.27560330509981e-10	1.00300835606217e-06	5.66130204417198e-09
185	3.07503064880125e-10	1.00300835606217e-06	5.36961557606743e-09
186	3.46791589450593e-10	1.00300835606217e-06	5.64778147113360e-09
187	3.45723319708938e-10	1.00300835606217e-06	5.33252765556740e-09
188	2.44085301199266e-10	1.00300835606217e-06	5.84562879585280e-09
189	2.97937492620701e-10	1.00300835606217e-06	5.06573110167355e-09
190	3.08276708284941e-10	1.00300835606217e-06	5.02451683762555e-09
191	6.49212136535213e-10	1.00300835606217e-06	5.58224997918592e-09
192	3.60997801335745e-10	1.00300835606217e-06	5.95363186874659e-09
193	3.34922630737886e-10	1.00300835606217e-06	5.77848632446579e-09
194	3.82245551328880e-10	1.00300835606217e-06	5.97977480032533e-09
195	3.19654908278379e-10	1.00300835606217e-06	5.31570429373783e-09
196	4.18187019815155e-10	1.00300835606217e-06	5.50791627784073e-09
197	3.43554254421990e-10	1.00300835606217e-06	5.80184363412237e-09
198	4.38909783951826e-10	1.00300835606217e-06	5.45134557607216e-09
199	3.22194045150551e-10	1.00300835606217e-06	5.77271134073000e-09
200	2.48820649297845e-10	1.00300835606217e-06	5.81138637565604e-09

==> experiments/quadraticpow2.tex <==
n err bound boundsharp
1	2.50283765134306e-08	0.0141460905349794	9.53184955631222e-07
2	1.90995023002329e-08	0.0141460905349794	1.12812522390651e-06
3	2.00622309177503e-08	0.00437709973009027	5.58356756608331e-07
4	1.84934297470399e-08	0.00210471306258390	3.72911106502349e-07
5	1.32356353643424e-08	0.00123353682278243	2.91810605687304e-07
6	1.31981509450575e-08	0.000809638105179936	2.02621084141936e-07
7	9.39707523894521e-09	0.000571934551370692	1.78690682493310e-07
8	6.70430665253506e-09	0.000425410068499827	1.60523224796101e-07
9	1.28006148338761e-08	0.000328754498501940	1.40204308945680e-07
10	8.04708403790462e-09	0.000261657982225811	1.23074947338683e-07
11	1.13219283344857e-08	0.000213189101188225	1.15771337816680e-07
12	6.51523463223091e-09	0.000177039759861924	1.00248493121288e-07
13	5.10031377887612e-09	0.000149362631715207	9.94331525773908e-08
14	4.79395822687316e-09	0.000127702988623400	8.69243524500956e-08
15	5.52112775039484e-09	0.000110434826674932	7.49083635920664e-08
16	4.77932393180974e-09	9.64464534181818e-05	8.13867448507776e-08
17	3.06133629975080e-09	8.49569336165779e-05	7.22384378544943e-08
18	4.48021086626240e-09	7.54046557344596e-05	6.36998902834390e-08
19	2.93398339524497e-09	6.73773610834589e-05	6.27639131203686e-08
20	3.76296532318484e-09	6.05668969613568e-05	5.93033716691927e-08
21	2.80217007983064e-09	5.47391909155145e-05	5.57291848045537e-08
22	2.83328862586744e-09	4.97138633861360e-05	5.17838423437578e-08
23	3.08647900793004e-09	4.53500982756422e-05	4.82859069750154e-08
24	2.60808176437999e-09	4.15366686358043e-05	5.22801576379303e-08
25	2.68910282684228e-09	3.81847774506514e-05	4.88928751573555e-08
26	3.52389759363339e-09	3.52228407797636e-05	4.68393255391517e-08
27	2.61606410923965e-09	3.25926335280430e-05	4.71802334451314e-08
28	1.43562575818715e-09	3.02464057510954e-05	4.08383893881235e-08
29	1.78938279144492e-09	2.81446999137020e-05	3.96181889877761e-08
30	3.40057043300171e-09	2.62546809267886e-05	3.80884991833153e-08
31	2.87454804142774e-09	2.45488457700724e-05	3.77909668175528e-08
32	2.04647282019106e-09	2.30040172019887e-05	3.84381995515560e-08
33	1.64728039035514e-09	2.16005522619753e-05	3.66942455415931e-08
34	2.10100059957094e-09	2.03217147217311e-05	3.28433274990883e-08
35	2.37633634284197e-09	1.91531737916964e-05	3.55568932792154e-08
36	1.66722444190061e-09	1.80826008656139e-05	3.15334834560588e-08
37	1.41324140393840e-09	1.70993429874790e-05	3.01923988247863e-08
38	1.07322066152361e-09	1.61941568008078e-05	3.09125544310493e-08
39	1.27643896298605e-09	1.53589905075740e-05	3.15900490137794e-08
40	1.20480788367016e-09	1.45868041849405e-05	2.96153829517311e-08
41	6.34699067062628e-10	1.38714209372779e-05	2.64447581565927e-08
42	2.04812744087980e-09	1.32074029808587e-05	2.62636251173085e-08
43	1.05139990310684e-09	1.25899480000051e-05	2.72967666512020e-08
44	9.38995546118468e-10	1.20148020713982e-05	2.60772920294002e-08
45	2.14860279274791e-09	1.14781861973416e-05	2.69369568166321e-08
46	1.57452942153921e-09	1.09767340703737e-05	2.32633474563494e-08
47	1.13253236019061e-09	1.05074391489324e-05	2.49088163548120e-08
48	1.25575519427112e-09	1.00676094854020e-05	2.42412737848028e-08
49	1.36416532886756e-09	9.65482903538334e-06	2.52145388459496e-08
50	7.47499208633567e-10	9.26692440680017e-06	2.31574477149944e-08
51	7.25119270786332e-10	8.90193619198304e-06	2.16480613227891e-08
52	8.44966891241147e-10	8.55809417477953e-06	2.25386101487432e-08
53	1.20846354824576e-09	8.23379582543359e-06	2.18243716028811e-08
54	1.34046192869267e-09	7.92758759423699e-06	2.20318303313641e-08
55	7.32628169145659e-10	7.63814859528141e-06	2.14714975859527e-08
56	1.06523273058896e-09	7.36427633756696e-06	1.94175518951190e-08
57	1.16708322356166e-09	7.10487421504242e-06	2.05283788387603e-08
58	1.06855864827490e-09	6.85894051207139e-06	2.09101070983081e-08
59	1.21249823869256e-09	6.62555871809761e-06	2.05062206047960e-08
60	7.40032418308950e-10	6.40388897632632e-06	1.85168184126130e-08
61	7.91936033446003e-10	6.19316051717550e-06	1.73633710054087e-08
62	8.12945227619758e-10	5.99266494899010e-06	1.98193830288339e-08
63	7.62815254618497e-10	5.80175029678941e-06	1.66852384573366e-08
64	8.90419790240822e-10	5.61981569522930e-06	1.81375333210116e-08
65	6.05930164568880e-10	5.44630665499425e-06	1.75953227317454e-08
66	9.12118683565956e-10	5.28071083288560e-06	1.86231334813766e-08
67	7.20584112592477e-10	5.12255424527005e-06	1.72098756007568e-08
68	5.52786206855594e-10	4.97139787256283e-06	1.74884731027739e-08
69	9.13672691720180e-10	4.82683460926654e-06	1.54906514984659e-08
70	8.74502409187788e-10	4.68848651995169e-06	1.69289693196529e-08
71	6.41204619800128e-10	4.55600236660191e-06	1.62301923857531e-08
72	5.29844034914503e-10	4.42905537708153e-06	1.52314056382569e-08
73	6.87422907859079e-10	4.30734122822297e-06	1.55491059792681e-08
74	7.29958441750920e-10	4.19057622026390e-06	1.47882132820045e-08
75	4.84318760644822e-10	4.07849562216464e-06	1.54104765801423e-08
76	9.73597005930260e-10	3.97085216976706e-06	1.40795830157420e-08
77	5.43838170975409e-10	3.86741470087074e-06	1.54227396453195e-08
78	1.24252258689464e-09	3.76796691314446e-06	1.41893619956534e-08
79	8.55812835746895e-10	3.67230623239994e-06	1.46448606529147e-08
80	3.77830624235764e-10	3.58024278016146e-06	1.43232863275062e-08
81	4.90964719880261e-10	3.49159843069832e-06	1.59984993417693e-08
82	9.27166025352456e-10	3.40620594876874e-06	1.49459050337604e-08
83	5.34690345024223e-10	3.32390820027544e-06	1.33843164644035e-08
84	4.48199760219563e-10	3.24455742887106e-06	1.45540730404915e-08
85	6.04304896896227e-10	3.16801459229033e-06	1.40172847559779e-08
86	5.38161338864367e-10	3.09414875283906e-06	1.29159134483955e-08
87	5.46772295943516e-10	3.02283651704748e-06	1.26817042126852e-08
88	5.89537861929687e-10	2.95396152000749e-06	1.34289028123498e-08
89	3.54693021710466e-10	2.88741395036729e-06	1.24751492516140e-08
90	4.58072528191194e-10	2.82309011236076e-06	1.28471288716541e-08
91	3.84663748702487e-10	2.76089202160797e-06	1.29231870510461e-08
92	7.49685532174871e-10	2.70072703174324e-06	1.25682365233201e-08
93	4.12569677427025e-10	2.64250748921257e-06	1.24649706523172e-08
94	5.02188682500190e-10	2.58615041383775e-06	1.25176697424133e-08
95	2.55166640413941e-10	2.53157720297201e-06	1.10607156012609e-08
96	7.25013932472115e-10	2.47871335727706e-06	1.18679093128299e-08
97	6.83726064103165e-10	2.42748822633405e-06	1.20840692157400e-08
98	4.69675673788906e-10	2.37783477246597e-06	1.15409678574803e-08
99	5.10736801370499e-10	2.32968935129643e-06	1.22907709796368e-08
100	2.97164483538985e-10	2.28299150770308e-06	1.16657979667128e-08
101	4.15767860458555e-10	2.23768378594357e-06	1.16501130609856e-08
102	8.14628683563786e-10	2.19371155284025e-06	1.07859836070217e-08
103	3.70670036416366e-10	2.15102283300694e-06	1.09627407697017e-08
104	4.39985643038363e-10	2.10956815518974e-06	1.21544716654913e-08
105	4.38193943481740e-10	2.06930040887321e-06	1.07131079279870e-08
106	3.54051023841479e-10	2.03017471037553e-06	1.06293493990280e-08
107	2.36364436941341e-10	1.99214827772193e-06	1.03636119423276e-08
108	4.73565660537829e-10	1.95518031364453e-06	1.12588947325167e-08
109	4.08121500409365e-10	1.91923189611123e-06	1.05386633795296e-08
110	6.45486210809896e-10	1.88426587583488e-06	1.03415150067715e-08
111	2.22324787543410e-10	1.85024678025857e-06	9.25913547403843e-09
112	2.77712779274165e-10	1.81714072355370e-06	1.00212309809581e-08
113	3.47234765580230e-10	1.78491532220425e-06	9.95600332915206e-09
114	4.04897783406060e-10	1.75353961578448e-06	1.02737571579815e-08
115	6.01952790742461e-10	1.72298399256807e-06	9.74272851328683e-09
116	2.80172353113860e-10	1.69322011963492e-06	9.70944185531253e-09
117	2.69725466330624e-10	1.66422087716747e-06	9.49505282379746e-09
118	3.48765942821901e-10	1.63596029665196e-06	9.02602673926604e-09
119	3.98927854197215e-10	1.60841350272163e-06	9.16966142953838e-09
120	3.27243783830453e-10	1.58155665839868e-06	8.57342371737116e-09
121	2.58371989685457e-10	1.55536691350980e-06	9.44056661295925e-09
122	4.34176583026156e-10	1.52982235606679e-06	9.56236492655285e-09
123	2.36523955995537e-10	1.50490196641914e-06	9.56980378963011e-09
124	5.18278342292137e-10	1.48058557399936e-06	1.01104911236443e-08
125	3.34314791638418e-10	1.45685381649484e-06	9.08653756373046e-09
126	3.69890150070574e-10	1.43368810129191e-06	9.23652201353619e-09
127	4.16354475407016e-10	1.41107056904876e-06	9.32725328075237e-09
128	1.69115154071423e-10	1.38898405926384e-06	8.07703168253441e-09
129	5.84395551633972e-10	1.36741207771592e-06	9.21464077192296e-09
130	3.69043425147667e-10	1.34633876566027e-06	9.25155833325497e-09
131	2.81247731206005e-10	1.32574887067368e-06	8.68576051967999e-09
132	2.24899735402645e-10	1.30562771904815e-06	8.81516001370906e-09
133	3.42913634175848e-10	1.28596118963996e-06	8.17936229980925e-09
134	4.49771612444197e-10	1.26673568908706e-06	8.36852210880168e-09
135	3.66628060458401e-10	1.24793812831363e-06	7.89511084004621e-09
136	3.72101236242217e-10	1.22955590024588e-06	7.74702137370182e-09
137	2.89939445659781e-10	1.21157685866837e-06	8.37926564001080e-09
138	2.75861326735416e-10	1.19398929815446e-06	8.21874729726455e-09
139	2.64486664836995e-10	1.17678193500914e-06	8.89622671383412e-09
140	4.98258034820142e-10	1.15994388916620e-06	8.93377095668937e-09
141	2.61607603091101e-10	1.14346466698551e-06	8.00767879033623e-09
142	4.74981624962345e-10	1.12733414489967e-06	7.68778687340596e-09
143	5.31618211819835e-10	1.11154255386240e-06	7.87287665128823e-09
144	2.53039084423120e-10	1.09608046455408e-06	7.96926752582998e-09
145	2.59806514418536e-10	1.08093877330259e-06	7.66219980378213e-09
146	2.29976210423791e-10	1.06610868868021e-06	8.08159076332591e-09
147	5.29660549362781e-10	1.05158171873968e-06	7.83129851854350e-09
148	3.63887403924390e-10	1.03734965885495e-06	7.74782408231286e-09
149	4.76560147379765e-10	1.02340458013395e-06	8.15676532021077e-09
150	2.19491782111359e-10	1.00973881837287e-06	6.89688862175791e-09
151	2.86570289687204e-10	9.96344963523353e-07	7.20033106489123e-09
152	2.26527866799267e-10	9.83215849645365e-07	7.61130568568868e-09
153	3.32430281567640e-10	9.70344545320417e-07	6.71017256158005e-09
154	6.18406964729302e-10	9.57724344501208e-07	6.97038846962727e-09
155	3.23824529112622e-10	9.45348757775077e-07	7.15347970439842e-09
156	3.34035365466487e-10	9.33211504020042e-07	7.28275544236699e-09
157	1.71439774675191e-10	9.21306502433388e-07	7.38257698722546e-09
158	3.30452045846450e-10	9.09627864913916e-07	7.24825980824432e-09
159	2.83785000190368e-10	8.98169888780025e-07	7.88881738509860e-09
160	3.17088515655059e-10	8.86927049806831e-07	7.57744547694323e-09
161	2.84028227282177e-10	8.75893995566425e-07	7.43827064955052e-09
162	2.64260957571519e-10	8.65065539056301e-07	7.65136522251682e-09
163	2.71039034367569e-10	8.54436652601771e-07	7.30748974919908e-09
164	2.91334028050796e-10	8.44002462019010e-07	6.32792951634420e-09
165	3.59509284215197e-10	8.33758241026045e-07	6.95350154533255e-09
166	3.92706366072684e-10	8.23699405889756e-07	6.80731368468752e-09
167	3.42546607857985e-10	8.13821510297537e-07	6.49122899826181e-09
168	4.69951948298856e-10	8.04120240442934e-07	6.83358089368119e-09
169	3.87954128056196e-10	7.94591410315095e-07	6.37162660291618e-09
170	2.78340283927405e-10	7.85230957182438e-07	7.39581361975220e-09
171	7.74076601338042e-10	7.76034937261441e-07	7.25918929155656e-09
172	5.22344237985485e-10	7.66999521561926e-07	7.32360665985828e-09
173	4.82550492892549e-10	7.58120991900671e-07	5.54745941291376e-09
174	6.29338307128016e-10	7.49395737075599e-07	7.48621249880779e-09
175	2.50528162406523e-10	7.40820249193191e-07	6.74320539486012e-09
176	3.28217083385007e-10	7.32391120142152e-07	6.56502600505158e-09
177	7.40012629456077e-10	7.24105038206716e-07	6.81409737102055e-09
178	4.55941598434164e-10	7.15958784813294e-07	6.46173909145489e-09
179	2.40608866910729e-10	7.07949231404515e-07	6.13806344807139e-09
180	3.09113176559922e-10	7.00073336434974e-07	6.46294380045348e-09
181	5.69409902343833e-10	6.92328142483314e-07	6.05973236684859e-09
182	4.40397439644663e-10	6.84710773475516e-07	6.51916923264824e-09
183	4.68449544465650e-10	6.77218432014526e-07	5.76435132176008e-09
184	4.67844604764838e-10	6.69848396811609e-07	6.65827260872477e-09
185	4.91260727727567e-10	6.62598020214990e-07	6.14229818157396e-09
186	6.52533639237850e-10	6.55464725831637e-07	5.67525157181920e-09
187	6.03563837102553e-10	6.48446006238158e-07	6.15686330061096e-09
188	3.26609072605953e-10	6.41539420777036e-07	6.17259479362230e-09
189	4.85759161990770e-10	6.34742593434583e-07	6.32449660616024e-09
190	3.62473383955663e-10	6.28053210797167e-07	6.54085055422207e-09
191	6.39471372815003e-10	6.21469020082419e-07	6.54175844744972e-09
192	6.36193452374644e-10	6.14987827242317e-07	5.71649440371255e-09
193	3.70142396905677e-10	6.08607495135139e-07	5.93819718756567e-09
194	4.02304559232791e-10	6.02325941763451e-07	5.93614429160788e-09
195	3.66752509953094e-10	5.96141138575427e-07	5.90871082080177e-09
196	5.52976877821731e-10	5.90051108826900e-07	6.10612515308544e-09
197	2.02444941014176e-10	5.84053926001677e-07	5.89039098341647e-09
198	4.02570965734008e-10	5.78147712287770e-07	6.06519860105176e-09
199	5.10208331999625e-10	5.72330637107284e-07	5.42974453238908e-09
200	2.64928817203340e-10	5.66600915697814e-07	6.23309870292413e-09

==> experiments/quadraticsqrroot.tex <==
n err bound boundsharp
1	1.07501995155992e-08	5.87092528750637e-06	2.12817603014266e-07
2	1.60427904658439e-08	9.99323753539758e-06	2.63842527183926e-07
3	1.83287652751220e-08	1.40857787202420e-05	2.86304478944660e-07
4	2.64302035898800e-08	1.81750259641600e-05	3.64711826536565e-07
5	3.34189271495104e-08	2.22671261995269e-05	4.06110867256648e-07
6	3.65355085411601e-08	2.63640170106037e-05	4.36225038862408e-07
7	3.58626667842404e-08	3.04663540220763e-05	4.68268341356127e-07
8	5.05621350408256e-08	3.45743191825779e-05	4.87115370363553e-07
9	2.62745349789683e-08	3.86879003123585e-05	4.97778849279062e-07
10	4.72785364581911e-08	4.28070023877921e-05	5.87653869093923e-07
11	5.08860150047123e-08	4.69314961186943e-05	5.89917577992362e-07
12	3.78733056701050e-08	5.10612404305578e-05	6.41539706648495e-07
13	4.93297065988025e-08	5.51960931859846e-05	6.41607009501715e-07
14	5.43271902018725e-08	5.93359162900112e-05	6.46110538654402e-07
15	3.97574722303106e-08	6.34805780031978e-05	7.22226736178953e-07
16	4.95161872633701e-08	6.76299538321486e-05	6.95918685986862e-07
17	3.71424114973299e-08	7.17839266899661e-05	7.37584737246008e-07
18	5.20052665596816e-08	7.59423866877135e-05	7.71273217694332e-07
19	6.87553038270488e-08	8.01052307491680e-05	8.52414187153447e-07
20	4.27241587119091e-08	8.42723621522384e-05	8.84301135413647e-07
21	4.88839791795716e-08	8.84436900526002e-05	8.32053693886229e-07
22	6.29586367090969e-08	9.26191290186633e-05	8.83761331005378e-07
23	3.31797607119942e-08	9.67985985923930e-05	9.06344040900639e-07
24	5.82004935757856e-08	0.000100982022882397	8.78786991548317e-07
25	6.07515375504940e-08	0.000105169330191073	8.36976367890757e-07
26	4.93029134604829e-08	0.000109360452675251	8.54843476043510e-07
27	8.04289607860479e-08	0.000113555326038527	9.59906839761434e-07
28	3.55606987321140e-08	0.000117753889252807	8.76081266860442e-07
29	5.21345489419644e-08	0.000121956084306511	8.58819234739403e-07
30	7.63469693058043e-08	0.000126161855976870	1.02900844086866e-06
31	4.51954457998674e-08	0.000130371151623796	9.56505613154203e-07
32	6.50500990332129e-08	0.000134583921003196	1.03570972200918e-06
33	5.01809083571083e-08	0.000138800116097527	1.00164552669538e-06
34	9.17421990868680e-08	0.000143019690961929	1.15482478458429e-06
35	4.43712441507672e-08	0.000147242601584113	1.13240023902257e-06
36	5.14378592447214e-08	0.000151468805756701	1.05995940035642e-06
37	6.73987477899501e-08	0.000155698262960605	1.04861146309428e-06
38	3.79434395169032e-08	0.000159930934258371	1.04031722616318e-06
39	3.14838726188573e-08	0.000164166782196443	1.06658510187760e-06
40	6.13353246374871e-08	0.000168405770715426	1.10921506809156e-06
41	7.26437099920820e-08	0.000172647865067596	1.14059156962430e-06
42	4.04076762510138e-08	0.000176893031740949	1.13572085646908e-06
43	4.60630506641666e-08	0.000181141238389064	1.19225284167227e-06
44	3.80939461918567e-08	0.000185392453766396	1.26924892726986e-06
45	6.76801173654857e-08	0.000189646647668322	1.20418528325039e-06
46	4.62344391777790e-08	0.000193903790875600	1.17522449185538e-06
47	4.21143251481120e-08	0.000198163855102856	1.19847767400437e-06
48	8.66655903724076e-08	0.000202426812950655	1.39724461197335e-06
49	5.64195382058781e-08	0.000206692637860941	1.27071061136710e-06
50	4.56045544262309e-08	0.000210961304075470	1.32555768188247e-06
51	5.01798720421009e-08	0.000215232786597060	1.28961689399341e-06
52	7.32408068313087e-08	0.000219507061153346	1.22823731271241e-06
53	4.44713026473907e-08	0.000223784104162949	1.32293212857306e-06
54	6.40559085780807e-08	0.000228063892703713	1.35087373272881e-06
55	2.46240796676460e-08	0.000232346404482951	1.37270551939807e-06
56	6.95989531570598e-08	0.000236631617809554	1.33020367385495e-06
57	5.26161377471832e-08	0.000240919511567754	1.34149705484563e-06
58	3.16917700778991e-08	0.000245210065192443	1.37165010997724e-06
59	6.10901585554752e-08	0.000249503258645913	1.28022276292673e-06
60	3.18025532984391e-08	0.000253799072396063	1.45190120474371e-06
61	4.11048975068877e-08	0.000258097487395600	1.41734216657304e-06
62	7.28467156153700e-08	0.000262398485062697	1.61363278466717e-06
63	4.91043406825633e-08	0.000266702047262453	1.32648435209391e-06
64	4.70673809766757e-08	0.000271008156289503	1.53299986303074e-06
65	3.85444915375252e-08	0.000275316794851523	1.34510004380180e-06
66	5.99740324259574e-08	0.000279627946053647	1.47122137688249e-06
67	9.26859185804434e-08	0.000283941593383533	1.61213610974449e-06
68	8.43457521550383e-08	0.000288257720697399	1.60559469160605e-06
69	5.02551878529409e-08	0.000292576312206646	1.54275909304538e-06
70	4.96620682179175e-08	0.000296897352465154	1.45409286672956e-06
71	4.17014507668789e-08	0.000301220826357239	1.38830004124383e-06
72	8.86108594467562e-08	0.000305546719086096	1.52323886638637e-06
73	6.02487293556517e-08	0.000309875016162992	1.49311383460842e-06
74	3.10483389156035e-08	0.000314205703396748	1.44934793821224e-06
75	6.63800090662843e-08	0.000318538766883834	1.61400531433884e-06
76	4.05952173447066e-08	0.000322874192998859	1.63704047269899e-06
77	1.00017437772159e-07	0.000327211968385564	1.69108279909657e-06
78	3.75663077189589e-08	0.000331552079948197	1.71336280491578e-06
79	3.05671166374631e-08	0.000335894514843118	1.72015683825518e-06
80	7.35570572650715e-08	0.000340239260471125	1.60194868829368e-06
81	7.92866620956970e-08	0.000344586304469626	1.67825067120794e-06
82	4.76830793486026e-08	0.000348935634705651	1.69487987751871e-06
83	5.47591207770847e-08	0.000353287239268710	1.63453869720118e-06
84	9.92440193109486e-08	0.000357641106464269	1.75264005294763e-06
85	4.23509677698851e-08	0.000361997224807371	1.71723849940149e-06
86	3.50915939488732e-08	0.000366355583016479	1.70452523066342e-06
87	4.41241687260378e-08	0.000370716170007636	1.67533698829675e-06
88	8.62667439812133e-08	0.000375078974888812	1.71456815822334e-06
89	9.08119031680582e-08	0.000379443986954471	1.83763572687130e-06
90	4.43899474830597e-08	0.000383811195680526	1.70111556357050e-06
91	6.37755969579834e-08	0.000388180590719067	1.75234849684297e-06
92	4.62727092019743e-08	0.000392552161893760	1.90590989617755e-06
93	5.12065995456537e-08	0.000396925899195197	1.74697051906852e-06
94	7.59572291859485e-08	0.000401301792776365	1.73011610658037e-06
95	4.18218294773662e-08	0.000405679832948283	1.62531445337523e-06
96	4.58883928895991e-08	0.000410060010176133	1.83611088887617e-06
97	4.66667709318224e-08	0.000414442315074999	1.80682334297884e-06
98	5.40105669660812e-08	0.000418826738406197	1.81587421888753e-06
99	1.22918847085603e-07	0.000423213271073417	1.84131701053907e-06
100	6.44997893650780e-08	0.000427601904119306	1.79831300455508e-06
101	4.87403523401566e-08	0.000431992628721880	1.91173255012044e-06
102	5.68085421814809e-08	0.000436385436191273	1.96536397757254e-06
103	5.77342023200302e-08	0.000440780317966503	1.85555384622639e-06
104	5.94804801767806e-08	0.000445177265612285	1.87947389139811e-06
105	6.93719050246000e-08	0.000449576270816134	1.89748490261239e-06
106	4.33647173387071e-08	0.000453977325385405	1.84400196763372e-06
107	4.69588608170696e-08	0.000458380421244439	1.83123469255519e-06
108	1.11808741364836e-07	0.000462785550431846	1.86511419331632e-06
109	4.42614302712290e-08	0.000467192705098008	1.90252348364503e-06
110	6.87284385703135e-08	0.000471601877502307	2.10941086689014e-06
111	7.10623319885321e-08	0.000476013060010801	1.94342698288670e-06
112	5.96011524948814e-08	0.000480426245093894	2.03906281608195e-06
113	1.52906091938232e-07	0.000484841425323779	2.20487692496990e-06
114	3.83521638726601e-08	0.000489258593372384	2.01374734588909e-06
115	8.06878644068798e-08	0.000493677742009153	2.16567806122242e-06
116	5.30539448709436e-08	0.000498098864098906	2.12411097670142e-06
117	5.64020996295092e-08	0.000502521952599927	1.97240709631313e-06
118	8.43436243049776e-08	0.000506947000561585	1.90792101256897e-06
119	9.59798275395337e-08	0.000511374001122892	1.94551688746693e-06
120	6.19508074362347e-08	0.000515802947510408	1.95375417815747e-06
121	9.14056690254890e-08	0.000520233833036290	1.99649121125101e-06
122	4.95764513905532e-08	0.000524666651096786	2.05588460781278e-06
123	5.46885088671694e-08	0.000529101395170358	2.10919645257131e-06
124	5.18883562128238e-08	0.000533538058815905	2.00328932773959e-06
125	1.07800580233743e-07	0.000537976635671623	2.16548149718616e-06
126	5.05214322553915e-08	0.000542417119452765	1.97444771478116e-06
127	5.60701860942916e-08	0.000546859503950485	2.02402874595749e-06
128	1.12417414492584e-07	0.000551303783030599	2.19773288648305e-06
129	4.81461830265065e-08	0.000555749950631409	2.11432555655311e-06
130	1.32147659848445e-07	0.000560198000762954	2.15037663443374e-06
131	1.07400240576987e-07	0.000564647927505499	2.29147459556591e-06
132	6.23658277417176e-08	0.000569099725007807	2.05496621590344e-06
133	1.55344356584100e-07	0.000573553387486462	2.00048463430533e-06
134	8.99035058388612e-08	0.000578008909223997	2.29324043658814e-06
135	8.40455829898425e-08	0.000582466284568069	2.21482809739364e-06
136	7.62773983582224e-08	0.000586925507930225	2.36070286593765e-06
137	7.03525640985938e-08	0.000591386573784459	2.19933260896521e-06
138	5.73094212112930e-08	0.000595849476666251	2.30639403219174e-06
139	1.32321776486643e-07	0.000600314211171560	2.37732412834068e-06
140	6.43732529607628e-08	0.000604780771955662	2.33812011788991e-06
141	1.09017428982158e-07	0.000609249153731837	2.21469187586652e-06
142	9.77378924915358e-08	0.000613719351270749	2.43962615297810e-06
143	1.07678098920403e-07	0.000618191359399263	2.30030973479065e-06
144	9.58245869998886e-08	0.000622665172999282	1.98751776224591e-06
145	8.34784526497606e-08	0.000627140787007141	2.02187872245916e-06
146	9.06127985949569e-08	0.000631618196412389	2.44273185571602e-06
147	1.32764321126265e-07	0.000636097396256981	2.49844080658388e-06
148	6.43636418038426e-08	0.000640578381634416	2.39675920911274e-06
149	8.11508600256283e-08	0.000645061147688811	2.13544901764867e-06
150	1.31269459134212e-07	0.000649545689614148	2.31471722721193e-06
151	1.13548672041337e-07	0.000654032002653320	2.44261135394118e-06
152	1.23082145712700e-07	0.000658520082097242	2.44549167045593e-06
153	7.88729576695679e-08	0.000663009923284409	2.26227222045055e-06
154	1.98776946328522e-07	0.000667501521599898	2.38783790422160e-06
155	9.59950064488838e-08	0.000671994872474399	2.20497194103326e-06
156	1.53581039347741e-07	0.000676489971383905	2.52434998865584e-06
157	1.56079032171092e-07	0.000680986813848646	2.61601186217575e-06
158	9.94991999141922e-08	0.000685485395432696	2.15555527747251e-06
159	1.57271290676866e-07	0.000689985711742832	2.59859104753775e-06
160	1.24312369602156e-07	0.000694487758428470	2.51382185576681e-06
161	6.82496239786522e-08	0.000698991531180285	2.50389048340361e-06
162	6.97623012910335e-08	0.000703497025730265	2.43141296976428e-06
163	1.47612723504450e-07	0.000708004237850553	2.34871828488890e-06
164	1.61109104052714e-07	0.000712513163353152	2.74731734032072e-06
165	1.07382246962942e-07	0.000717023798089168	2.62298056494358e-06
166	1.24846345423000e-07	0.000721536137948216	2.62546757427416e-06
167	1.47010353428444e-07	0.000726050178857840	2.34802853068570e-06
168	1.04582395312348e-07	0.000730565916783082	2.47057247553676e-06
169	4.73460283293029e-08	0.000735083347725680	2.42974130139949e-06
170	1.45512568175503e-07	0.000739602467723900	2.48781423662976e-06
171	7.39240910348480e-08	0.000744123272851468	2.26079990879120e-06
172	1.02463702947977e-07	0.000748645759217439	2.48584447706541e-06
173	1.43329553982773e-07	0.000753169922965769	2.51338395145258e-06
174	1.28546910265830e-07	0.000757695760274481	2.47293618814747e-06
175	1.88163912437989e-07	0.000762223267355212	2.37564807820681e-06
176	1.09314186411098e-07	0.000766752440453095	2.61597204405108e-06
177	1.12423922783054e-07	0.000771283275845802	2.74368096646739e-06
178	1.27861048510453e-07	0.000775815769843589	2.14646310741171e-06
179	1.82322785740111e-07	0.000780349918788195	2.41373758094867e-06
180	8.13543414905918e-08	0.000784885719053192	2.47853683743283e-06
181	1.36488926358970e-07	0.000789423167042636	2.63926319973912e-06
182	1.48902374479171e-07	0.000793962259191666	2.75511835210345e-06
183	1.19700303330755e-07	0.000798502991965122	2.51497990488669e-06
184	2.70102573308788e-07	0.000803045361857733	2.43061115303185e-06
185	9.28475239361027e-08	0.000807589365393659	2.40220113746662e-06
186	1.14344407023477e-07	0.000812134999125502	2.45813883816388e-06
187	2.18069800734335e-07	0.000816682259635151	2.80113199158599e-06
188	1.08860745708864e-07	0.000821231143531796	2.68088688504692e-06
189	1.17722576343812e-07	0.000825781647453131	2.59703750401292e-06
190	6.73126228356429e-08	0.000830333768063654	2.29775386791318e-06
191	1.47121478069939e-07	0.000834887502055412	2.62400516716445e-06
192	2.64146832922666e-07	0.000839442846146628	2.45763427450722e-06
193	1.08163526857496e-07	0.000843999797082317	2.92730758360342e-06
194	1.05306488618045e-07	0.000848558351633284	2.75107388682176e-06
195	1.21398656293275e-07	0.000853118506595883	2.48719703290842e-06
196	1.12214535393294e-07	0.000857680258792099	2.71638297200567e-06
197	4.20213798664048e-07	0.000862243605068543	2.83254303703578e-06
198	8.75369667925102e-08	0.000866808542296838	2.82013790251074e-06
199	2.70947114132395e-07	0.000871375067372910	2.60442760601265e-06
200	1.01097191395995e-07	0.000871375067372910	2.89846425543624e-06
